Contracts: A unified lens on congestion control robustness, fairness, congestion, and generality

Congestion control algorithms (CCAs) operate in partially observable environments, lacking direct visibility into link capacities, or competing flows. To ensure fair sharing of network resources, CCAs communicate their fair share through observable signals. For instance, Reno's fair share is encoded as $\propto 1/\sqrt{\texttt{loss rate}}$. We call such communication mechanisms \emph{contracts}. We show that the design choice of contracts fixes key steady-state performance metrics, including robustness to errors in congestion signals, fairness, amount of congestion (e.g., delay, loss), and generality (e.g., range of supported link rates). This results in fundamental tradeoffs between these metrics. Using properties of contracts we also identify design pitfalls that lead to starvation (extreme unfairness). We argue that CCA design and analysis should start with contracts to conscientiously pick tradeoffs and avoid pitfalls. We empirically validate our findings and discuss their implications on CCA design and network measurement.

==> sections/archive/acknowledgements.tex <==
%-------------------------------------------------------------------------------
\section*{Acknowledgments}
%-------------------------------------------------------------------------------

The USENIX latex style is old and very tired, which is why
there's no \textbackslash{}acks command for you to use when
acknowledging. Sorry.



==> sections/archive/availability.tex <==
%-------------------------------------------------------------------------------
\section*{Availability}
%-------------------------------------------------------------------------------

USENIX program committees give extra points to submissions that are
backed by artifacts that are publicly available. If you made your code
or data available, it's worth mentioning this fact in a dedicated
section.

==> sections/archive/background.tex <==
%-------------------------------------------------------------------------------
\section{Background and motivation}
\label{sec:background}
\label{sec:motivation}
% \label{sec:contracts}
%-------------------------------------------------------------------------------

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/assumptions-contract.drawio.pdf}
    \caption{\label{fig:assumptions-other-flows} Without making assumptions
    about other flows, the red flow cannot distinguish between the two
    scenarios.}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/contract.pdf}
    \caption{\label{fig:reno-contract} Reno uses loss rate to communicate fair
    shares}
\end{figure}

\myparagraph{Why do we need contracts?} CCAs do not know how many flows they
are competing against. As a result, without any agreement between flows, they
cannot know their fair share.
% CCAs operate under partial observability. They may not know the network link
% rate, topology, routing, how many flows they compete against, or what CCA
% other flows may be using. To fairly allocate rates, CCAs need to make
% assumptions about other flows. At minimum, they assume that other flows are
% not blindly blasting packets.\va{since congestion control is a cooperative
% game} Typically, CCAs have to make even stronger assumptions.
For instance, consider the scenarios in \autoref{fig:assumptions-other-flows}.
If the green (upper) flow in scenario B exactly emulates the cumulative effect
of the three green flows in scenario A, then the red flow cannot tell the
difference. Its observations (timestamps of when packets were sent and
acknowledged) are identical. Yet, its fair share is different.
% To reach fairness, the red flow assumes that the other flows are following
% the contract, \ie, the thick green flow will realize that it is violating the
% contract and reduce its rate.

Contracts help flows to disambiguate between the two scenarios. All flows agree
to follow an encoding of fair share into globally observed signals. For
example, Reno uses: ``$\texttt{rate} = \texttt{const}/\sqrt{\texttt{loss
rate}}$''~\cite{mathis-model, tfrc}. While this is not explicit in the
algorithm, the emergent behavior is that all flows measure the average packet
loss rate and calculate a \emph{target rate} using this formula. Then they
increase or decrease their actual sending rate to move towards the target.

% Assumptions about the other flows' behavior helps the flows to distinguish
% between the two scenarios. To reach fairness, flows encode their estimate of
% the fair-share into globally observed signals. For example, Reno~\cite{reno}
% encodes it in the loss rate~\cite{mathis-model,tfrc}: ``$\texttt{rate} =
% \texttt{const}/\sqrt{\texttt{loss rate}}$'', as illustrated in
% \autoref{fig:reno-contract}, and assumes that all other flows follow this
% relation. While this is not explicit in the algorithm, the emergent behavior
% is that all flows measure the average packet loss rate and calculate a
% \emph{target rate} using this formula. Then they increase or decrease their
% actual sending rate to move towards the target.

% Note, such assumptions are looser than knowing the full CCA of the other
% flows. \Eg, TFRC~\cite{tfrc} and some binomial congestion control
% algorithms~\cite{binomial-infocom} also use the same target rate but are
% otherwise different (\eg, in terms of stability and convergence times).

% We can interpret this relation as the target
% sending rate corresponding to the measured average loss event rate. On a
% dumbbell topology, all flows measure the same average loss event rate. If their
% current sending rate is above target, they reduce their sending rate,
% otherwise, they increase their rate. This way, in steady-state a fixed point is
% reached, \ie, all flows achieve the same average sending rate, and the sum of
% their average rates is equal to the bottleneck bandwidth\footnote{If the flows
% do not fully utilize the link, there would not be any queuing, and the flows
% would measure a loss event rate of zero and ramp up their rate.}, and the
% average loss rate stops changing.

Turning back scenario B in \autoref{fig:assumptions-other-flows}, both red and
green flows measure the same loss rate, and hence calculate the same target
rate, but they have different sending rates. Thus, at least one of them will
change their sending rate until they reach a steady-state where everyone's
sending rates are equal to the target rate.
% \va{These equilibrium points also defines the flavor of fairness for which
% the CCA is designed. Reno corresponds to weighted minimum potential delay
% fairness.} \anup{It's not the point, but the shape of contract.} \va{now?
% Changed "This equilibrium point" to "these equilibrium points"} \va{@Anup -
% .Everyone's rates are not equal and may not add up to the link rate right?
% That is why I modified your modification} \anup{In steady state all rates
% should be equal and add up to the link rate. Its a dumbbell topology.}
All existing CCAs (to our knowledge) use a similar method of coordination. The
signal used and the shape of contract changes, but the concept remains the
same.

% The only difference is in the globally observable signal that they use (\eg,
% loss rate, delay, ECN marking rate) and the function that determines the
% target rate. For example, Vegas~\cite{vegas,duality-vegas},
% FAST~\cite{fasttcp} and Copa~\cite{copa,starvation} use ``$\texttt{rate} =
% \texttt{const} / \texttt{delay}$'', where $\texttt{delay}$ is an estimate of
% the queuing delay = $\rtt - \min \rtt$. Note, throughout the paper by delay
% we mean the queuing delay estimate.

\noindent\textbf{Contracts in general.} A CCA contract takes the form
``$\texttt{average sending rate} = \func(\texttt{aggregate statistic})$'' and
describes the CCA's observations in steady state (\eg, at time infinity). In
short, we denote it as ``$\x = \func(\s)$''. Here, $\s$ can be any aggregate
statistic of the CCA's observations: the time series of sequence numbers of the
sent and acknowledged packets, and any explicit signals (\eg ECN) sent by the
network. Statistics like delay, loss and ack rate can be derived from these.

All CCAs have at least one contract since ``$\texttt{average sending rate} =
\texttt{average sending rate}$'' holds trivially. As described above, more
interesting contracts usually exist where our theorems offer non-trivial
insights. In principle, we can derive all the contracts a CCA satisfies by
running it on all possible network topologies to collect a large set of
steady-states described by the CCA's observations. Then we can group flows that
had the same sending rate and determine which aggregate statistics predict this
grouping. While this is uncomputable in theory, in practice useful contracts
are known for most CCAs. They are either computed while designing the CCA, or
by a post-hoc analysis. Thus, we focus on how the choice of contract impacts
performance metrics and the tradeoffs it creates.
\autoref{tab:contracts-summary} lists contracts for some CCAs. Examples of how
these are computed can be found in
literature~\cite{ecn-vs-delay,starvation,bbr-rate-contract,dctcp-analysis}.\va{I
have commented out a para on how these contracts are computed in literature and
replaced it with citations}

\anup{Computed using fluid anaysis. Contract representation works even when the
equilbirum is limit cycle instead of fixed point. Even if the CCA is
complicated its equilbrium can be modeled. \Eg, BBR in cwnd-limited does ..,
and rate limited does ...}

\if 0 These are often computed by analyzing CCAs in the fluid model and
computing the equilibrium behavior (for \eg, see~\cite{ecn-vs-delay}). It may
not be straightforward to build fluid models for complicated CCAs, but we can
still describe their equilibrium behavior. \Eg, BBR in cwnd-limited mode
encodes fair share in delay~\cite{starvation}, and in rate-limited mode encodes
information in ``growth in delivery rate during
probing''~\cite{bbr-rate-contract}. Further, the equilibrium behavior may be
different for different CCAs. \Eg, DCTCP~\cite{dctcp} has a limit cycle
equilibrium instead of a fixed-point equilibrium, we can represent limit-cycles
describing a cycle instead of a time instance, \eg, for DCTCP, ``$\texttt{cwnd}
= 1/(\texttt{average ECN marking rate})^2$''~\cite{dctcp-analysis, dctcp}.
\fi

\anup{If CCAs have same contract, implies they will be fair to each other.}

\noindent\textbf{Restrictions.} To generalize beyond NUM, we only study
dumbbell and parking lot topologies (see~\autoref{fig:parking_lot}) in this
paper. They are common in the WAN and datacenters. Further, any negative
results proved for these will also hold in a general network topology.\va{@Anup
- please check if the preceeding sentences make sense} Further, we only
consider contract functions that are strictly increasing\va{decreasing?} with a
closed domain range (and are hence continuous and invertible). All contracts
that we are aware of have this property since the aggregate statistic is a
measure of congestion (\eg loss or delay) and it is safer to reduce the sending
rate when congestion increases. Doing otherwise can cause the CCA's rate to
diverge.

% it cannot be the case that both the flows even if the red flow is at the
% correct target rate for the measured loss rate, the green flow would not be.
% \anup{It cannot be that both the flows are at target rate, they measure the
% same loss rate, but their rates are different.} The green flow will realize
% that it is sending above the target rate and reduce its rate to converge to a
% fair share.

% All existing CCAs use a similar method of coordination, \eg,
% Vegas's~\cite{vegas} and Copa's~\cite{copa} steady-state rate is of the form:
% ``$\texttt{rate} = \texttt{const}/\texttt{delay}$''. Where, delay is their
% estimate of the non-propagation delay component of the RTT. Different CCAs
% change the shape of the steady-state target rate function (\eg, inverse vs
% inverse square root, or, steeper vs. gradual) and the congestion signals used
% (\eg, loss rate, delay, ECN marking rate), but the coordination method is the
% same.

% \anup{TODO: merge this here or next section.

% We call the function that relates a CCA's steady-state rate to observed
% signals (or statistics derived from observed signals) as the contract. We
% think of contracts as the assumptions flows make about the actions of the
% other flows. Knowing that the other flows are following the contract, allows
% flows to disambiguate their fair share. Without such an agreement, it is hard
% for a CCA to infer how many flows they may be competing against or its fair
% share. Note that these assumptions are looser than knowing the full CCA of
% the other flows. \Eg, both TFRC~\cite{tfrc}, Reno (AIMD)~\cite{reno}, and a
% subset of binomial congestion control algorithms~\cite{binomial-infocom}
% share the same contract (and thus are fair to each other), but they are
% different CCAs (\eg, have different stability/convergence time properties).}

%-------------------------------------------------------------------------------
% Motivation from thesis proposal
%-------------------------------------------------------------------------------

% In \S\ref{sec:ccmatic} and \S\ref{sec:minimax} we only explored scenarios with
% one flow. In this section, we consider scenarios with multiple flows and
% explore design of CCAs that can ensure fair sharing of network resources or
% avoid starvation when network has jitter.
% % When we are doing this we assume that congestion control is trying to solve
% % the network resource allocation problem in a decentralized and cooperative
% % way. With centralized control, the controller knows what are the capacities
% % on the links ... By cooperative, we mean that the flows agree on a global
% % utility. We are not concerned with if flows with different local utilities
% % will agree on a global utility. The central solution works, can we get to the
% % same allocation in a decentralized way while dealing with feedback noise.
% If we want to apply techniques similar to \S\ref{sec:minimax}, we have to
% enumerate the game tree, this requires a way to not just speculate the actions
% the network may take but also speculate what the other flow's actions may be.
% We cannot share the network resources fairly with other flows if they can take
% arbitrary actions, and so we need to make assumptions about what actions they
% may take. \Eg, if the other flows just blast packets, then we cannot share the
% network fairly with them while still bounding congestion.

% One assumption we can make is that the other flows are using the same CCA as
% us, but this is the same CCA we are trying to synthesize, and it becomes a
% circular problem.  This circular problem can be represented as a cooperative
% multi-agent game, where flows are trying to cooperate and win against the
% network (as opposed to a non-cooperative game where flows are working against
% each other). We can also think of this as a Dec-POMDP (decentralized partially
% observable markov decision process). C.f. with our single-flow formulation
% which was a POMDP, \ie, without the decentralized part. Solving cooperative
% multi-agent problems is much harder than their non-cooperative equivalents, and
% unfortunately, we cannot use the same techniques as before. Solving general
% Dec-POMDPs is NEXP-complete, while solving general POMDPs is
% PSPACE-complete~\cite{decpomdp}.\footnote{PSPACE $\subsetneq$ NEXP, and P
% $\subseteq$ NP $\subseteq$ PSPACE. While it is known that PSPACE $\neq$ NEXP,
% it is not known if P = PSPACE or P $\subsetneq$ PSPACE (as of 2024).}

% There are exact ways to solve discrete Dec-POMDPs (\eg, dynamic
% programming~\cite{decpomdp}). These are similar to minimax
% (\S\ref{sec:minimax}) but additionally require enumerating possible policy
% trees of other players at each move to see feasible moves for other players.
% However, the number of policy trees is exponentially large in the trace
% lengths, and the exact techniques quickly become intractable as the problem
% size increases. To our knowledge Remy~\cite{remy} is the only past work that
% uses a Dec-POMDP formulation for CC. However, to make the problem tractable, it
% only explores a restricted search space of CCAs and network environments. Remy
% summarizes the history of observations in an ad-hoc way (\eg, average sending
% rate and average ACK rate) instead of exploring more general ways to derive
% statistics from the history of CCA's observations. It also does not explicitly
% consider networks with jitter.

% Given it is hard to practically use exact methods to solve Dec-POMDPs, we
% considered exploring domain specific heuristics to simplify the problem. We
% want to ease the computer's job of synthesizing congestion control by
% incorporating human-intuition. We investigated how existing CCAs achieve
% decentralized coordination to reach fair shares, and found that all existing
% CCAs use almost the same way to coordinate fair shares.

% ------------------------------------------------------------------------------

% We need to make assumptions about other flows to be able to speculate what
% might happen. The first assumption is are they non-cooperative or
% cooperative. If they are non-cooperative, then they can just steal bandwidth.

% If they are cooperative, then the problem is harder. The full assumption we
% make about the other flows is the policy they are using, but this is the same
% policy we want our agent to have. It is a circular problem.

% Set of all compatible policies.

% What do we need cooperation for. Inferring flow count or fair share. New
% abstraction called contract that aims to describe the method CCAs use to
% communicate fair shares. It can also be interpreted as an assumption about
% the other flows.

% \subsection{Dec-POMDPs}

% Multi-agent cooperative problems are much harder than non-cooperative problems.
% Cooperative problems are modeled as Dec-POMDPs (decentralized POMDPs).
% Multi-agent, non-cooperative problems can be solved as one vs. rest, and
% effectively formulated as POMDPs. However, we can't do this for cooperative
% problems. Solving general Dec-POMDP is NEXP-complete, while solving general
% POMDP is PSPACE-complete.\footnote{PSPACE $\subsetneq$ NEXP, and P $\subseteq$
% NP $\subseteq$ PSPACE. While it is known that PSPACE $\neq$ NEXP, it is not
% known if P = PSPACE or P $\subsetneq$ PSPACE (as of 2024).}

% There exist exact ways to solve discrete Dec-POMDPs. These are similar to
% minimax but additionally require enumerating possible policy trees of other
% players at each move to see feasible moves for other players. \anup{We did not
% explicitly explore this, but hunch is that this would be intractable.}
% \todo{Add summary from survey on Dec-POMDPs, and DP based exact ways of solving
% discrete Dec-POMDPs.}

==> sections/archive/contracts_old.tex <==
\section*{Contracts (old)}
\label{archive:sec:contracts}

\anup{Need better structure for this section. It feels like a laundry list of
caveats right now. Also, there are some redundancies in the intro/background
and contracts section that can be merged.}

% We are building an abstraction, called \textbf{contracts}, to formally
% describe methods to communicate fair shares. The hope is that this
% abstraction will allow is to understand both how the choice of contract
% affects performance, and how should we choose contracts to be robust to
% signal noise.

% \anup{Should we keep set of observations as the definition or just use the
% duality theory.}

% For now, we define a contract to be the same as the CCA's steady-state
% response function.

We call the function that relates a CCA's steady-state rate to observed signals
(or statistics derived from observed signals) as the contract. We think of
contracts as the assumptions flows make about the actions of the other flows.
Knowing that the other flows are following the contract, allows flows to
disambiguate their fair share. Without such an agreement, it is hard for a CCA
to infer how many flows they may be competing against or its fair share. Note
that these assumptions are looser than knowing the full CCA of the other flows.
\Eg, both TFRC~\cite{tfrc}, Reno (AIMD)~\cite{reno}, and a subset of binomial
congestion control algorithms~\cite{binomial-infocom} share the same contract
(and thus are fair to each other), but they are different CCAs (\eg, have
different stability/convergence time properties). \anup{TODO: Move the
assumptions part to motivation section, just keep contract does not fix CCA
part here. That too perhaps towards the end of the section.}

% Without such a contract, a flow cannot know its fair share. For example, ...
% This abstraction aims to capture the mechanism CCAs use to communicate their
% fair shares with each other.

% We found that the CCA's choice of contracts (or steady-state response
% function) fixes multiple different performance metrics a CCA achieves in
% steady-state. The different performance metrics require the contract function
% to take a different shape (\eg, steeper vs. more gradual function). As a
% result, a CCA cannot optimize for all the metrics at once. This led us to
% discover new impossibility results with regard to fairness in congestion
% control. These metrics include: (1) fairness when network have multiple
% congested hops (parking lot topology), (2) how congestion grows with the
% number of flows, (3) how robust is the CCA to errors in congestion signals,
% (4) what range of link rates a CCA supports.

% We currently define contracts as the steady-state response function of the CCA.
More formally, we define a contract as the set of observations (sending and
acknowledgment sequence number time series) of a CCA in steady-state (\eg, at
time infinity), when the CCA is competing with itself on a dumbbell or parking
lot topology (\autoref{fig:parking_lot}). Note that we also include a
time-series of explicit signals like ECN marks in the set of observations.

In principle, we can obtain this set for a given black-box CCA using the
following procedure. We run the CCA on dumbbell and parking lot topologies
competing with instances of itself. We repeat this for all possible choices of
flow count, link rate, propagation delay, and buffer sizes, and collect the
observations made by each flow at time infinity. The set of observations is the
contract. We can represent this set as a function but building equivalence
classes based on the average sending rate of the CCAs. All observations in an
equivalence class have the same sending rate and describe can describe the set
of equivalence classes in the form: ``\texttt{average sending rate} = \func
(\texttt{aggregate statistic derived from observation})''. As a shorthand, we
denote this form as ``$\x = \func(\s)$''. We refer to \func as the contract (or
contract function).

We describe the above procedure to illustrate the concept of contracts. In
practice, one would compute the contract for a CCA by analyzing its fluid model
and computing the equilibrium behavior, similar to the analysis
in~\cite{ecn-vs-delay}. We did not have to compute the contracts for CCAs
ourselves, as the steady-state behavior has already been analyzed for most
popular CCAs. Moreover, our focus is on how the choice of contract impacts
performance metrics and the tradeoffs it creates rather than
reverse-engineering contracts for CCAs.

Note, it may not be easy to build fluid models for complicated CCAs, but we can
still describe the equilibrium behavior of the CCA. \Eg, BBR in cwnd-limited
mode encodes fair share in delay~\cite{starvation}, and in rate-limited mode
encodes information in ``growth in delivery rate during
probing''~\cite{bbr-rate-contract}. Further, the equilibrium behavior may be
different for different CCAs. \Eg, DCTCP~\cite{dctcp} has a limit cycle
equilibrium instead of a fixed-point equilibrium, we can represent limit-cycles
describing a cycle instead of a time instance, \eg, for DCTCP,
``$\texttt{cwnd} = 1/(\texttt{average ECN marking rate})^2$''.

% (\eg, fixed-point, or limit cycles). Further, instead of trying to see what
% contracts CCAs follow, we start with assuming that the CCA follows a given
% contract, and then explore how this affects their performance metrics.


For simplicity, we only explore ``simple'' contracts. We discuss potential
extensions in \autoref{sec:limitations}.
% Set of observations in steady-state. Restrict to simple contracts See
% \autoref{app:contracts} for formal definition of contracts and more details.
% At a high level contracts help us solve the ``decentralized'' aspect of
% Dec-POMDPs. We assume other flows' actions follow some contract. This allows
% us to effectively convert a cooperative game theory problem into a
% non-cooperative problem: ``what is the action I should take to optimize my
% objective while still following the contract given that other flows are
% following the contract and the network is following the network model?''.
% Note, a contract need not fully specify the CCA (\eg, AIMD and TFRC follow
% the same contract (loss rate to sending rate mapping), but are different
% CCAs.). \anup{Also, currently, we are assuming other flows are following
% contract. Our current contract model does not study what happens when
% multiple flows are not in steady-state and as a result not following contract
% at the instant.}
A simple contract (set of steady-state observations) is one that can be written
in the form: ``\x = \func(\s)'', and,
\begin{packedenumerate}
    \item The aggregate statistic, \s, is one of the following: non-propagation
    delay (= RTT - min RTT) or simply delay (\eg, Vegas~\cite{vegas},
    Copa~\cite{copa}, Swift~\cite{swift}), average loss rate (\eg,
    Reno~\cite{reno,fairness-chiu-jain}, Cubic~\cite{cubic}), average ECN
    marking rate (\eg, DCTCP~\cite{dctcp}, DCQCN~\cite{dcqcn},
    MPRDMA~\cite{mprdma}), max per-hop delay (\eg, Poseidon~\cite{poseidon}),
    or bytes (or time) between high-delay (AIMD on delay,
    see~\autoref{sec:pitfalls}).
    \item The contract function, \func, is strictly monotonically decreasing
    (and so is also invertible).
    % \item CCA builds some queues in steady-state, so that utilization is
    % 100\%.
\end{packedenumerate}

Note, typically the statistic in the contract is a measure of congestion, \ie,
increasing the rate increases the statistic. As a result, an increasing
contract function would produce diverging behavior for such statistics. \Eg,
say a flow's rate is below target, and it increases its rate, then the
increased rate will increase the statistic, further increasing the target rate.
This cycle continues and the CCA diverges.

All known CCAs implicitly or explicitly choose a contract. This design choice
constrains/fixes various performance metrics.

\myparagraph{Contracts and NUM}
The concept of contracts can be described using the network utility
maximization (NUM)~\cite{num-kelly, num-srikant, num-low, num-low-book}
framework as well. Contracts describe the mapping between the congestion
measure (or price, aggregate statistic) and rate of the CCA. It is the same as
the demand function (target rate) for a given price~\cite{num-kelly}.
Alternatively, the inverse of a contract is the same as the link price (\eg,
target delay) for a given load (\eg, rate)~\cite{num-kelly}. Under this
correspondence, the utility function that the CCA optimizes is given by:
\begin{align}
    \utility(\x) = \int \func^{-1}(\x) \, d\x \label{eq:utility}
\end{align}
Where \utility is the utility that a flow derives from obtaining a rate of \x,
and \func is the contract. This derivation (done in \cite{num-low}) comes from
the fact that the points (\ie, $\langle \rate, \price \rangle$ pairs) that
satisfy the contract, also satisfy the Karush-Kuhn-Tucker (KKT) conditions of
the network utility maximization problem (\ie, maximize $\sum_i
\utility(\x[i])$, subject to link capacity constraints).

Note, \autoref{eq:utility} only holds if the statistic used in the contract
function adds up over links (\eg, delay adds up over hops). For other
statistics (\eg, max per-hop delay~\cite{poseidon}), the utility is different.

Given the similarity with the NUM literature, it is natural to ask what are the
new things we do. To our knowledge, the focus of the past work to understand
(or reverse-engineer) the equilibrium and stability properties of individual
CCAs. Instead of analyzing individual CCAs, we use contracts to effectively
parametrize the design space of CCAs to explore fundamental tradeoffs that any
CCA must face. \srini{should be in intro as well}

Depending on the reader, some of our findings may be seen as obvious deductions
from the NUM framework. \Eg, \cite{duality-vegas} shows coupling between
performance metrics for Vegas~\cite{vegas}. Despite that, the pitfalls we
describe were committed even after the NUM framework was popularized and
continue to be committed. Likewise, given there is a coupling between performance
metrics and contracts, ideally, the contract should be a direct consequence of
the desired objectives. Despite this, the contracts in new CCA design papers
are artifacts of other design choices rather than being conscientious decisions.

% The focus of the NUM literature was on understanding the performance of CCAs
% in steady-state. Our work is closely related to the NUM literature. It uses
% an optimization framework to reverse-engineer the utility functions of CCAs
% and understand their equilibrium properties. Instead, we treat the contracts
% as parameterization of the CCA design space, and then explore how...

% \anup{Many CCAs decide contract in an adhoc way, many times its just an
% artifact of other design choices rather than a conscientious decision.}

\todo{Is any of below not already conveyed that we may want to highlight in main text?}

\anup{Such derivations of metrics from contracts have actually been done
before~\cite{duality-vegas}. (1) Prior showed coupling exists for Vegas.
Coupling is more general. Obvious from past work, but tradeoffs not as
explicitly claimed or stated. (2) some of the metrics like operating range
start to matter more now (Internet is bigger than before), (3) pitfalls
(shifting, AIMD on delay, maxmin claim) while seemingly obvious were committed,
(4) broader set of signals (ideally all observations that can be derived).}

\anup{
Related work:
\\
Key difference is that we incorporate more questions, and make fewer
assumptions about the form. Interpret the theory to provide pitfalls to avoid.
Done by re-presenting the results. Naturally, target delay can shift but
utility can't shift, but since they are the same, target also cannot shift.
Many NUM approaches don't consider network diversity. Fairness metric paper
claims max-min fair CCA, but in the limit it only works on one network.
% \\
% Relation with NUM:
% 1. Kelly: primal target price - price, dual target rate source computation, or demand rate for a given price.
% 2. Duality: target rate. Under this interpretation, contract is the inverse of the derivative of utility.
}

==> sections/archive/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

==> sections/archive/intro-claude.tex <==
\section{Introduction}

Congestion control algorithms (CCAs) play a critical role in ensuring fair and efficient allocation of bandwidth in networks. Despite four decades of research asking fundamental questions—What is the best CCA? Do we need specialized CCAs or can we find one that fits many network scenarios? What are the fundamental limits of CCA performance?—the search for answers has remained elusive.

The challenge stems from CCAs operating in partially observable environments where they lack direct visibility into link capacities, network topology, or competing flows. To achieve fairness, CCAs must encode information about fair shares into observable network signals. For instance, Reno uses loss rate to coordinate fair shares, with each endpoint transmitting at an average rate $\propto 1/\sqrt{\text{loss rate}}$. We refer to such communication mechanisms as \emph{contracts}.

Traditionally, CCAs were designed to avoid congestion collapse, with fairness properties analyzed retrospectively~\cite{fairness-chiu-jain,num-srikant,num-low,num-kelly}. With the rise of applications like real-time communication and short remote-procedure calls (RPCs), newer CCA designs prioritized local performance metrics like latency and convergence time. However, this ``local'' perspective often led to undesirable fairness outcomes. For instance, TIMELY~\cite{timely} has been shown to have infinite fixed points, causing unfair rate allocations~\cite{ecn-vs-delay}.

\textbf{Our contributions.} We discover that the choice of contract—a design choice that may not have been made explicitly—fully determines four key congestion control metrics: (1) \emph{robustness} to noise in congestion signals, (2) \emph{fairness} in multi-bottleneck networks, (3) amount of \emph{congestion} (e.g., delay, loss), and (4) \emph{generality} (e.g., range of supported link rates). This leads to fundamental tradeoffs: robustness and fairness improve with gradual contracts, while congestion and generality improve with steeper contracts.

Using this contract-centered framework, we make three key contributions:

\textbf{First, we identify systematic mistakes in CCA design.} We discovered problems and tradeoffs in many modern CCAs including TIMELY~\cite{timely}, ICC~\cite{icc}, PowerTCP~\cite{powertcp}, and Poseidon~\cite{poseidon}. Our methodology works for analytically designed CCAs, implementations, and learned CCAs. We uncovered a bug in the Linux kernel implementation of TCP Vegas that has gone undetected for seven years and revealed weaknesses in Astraea~\cite{astrea}, a learned CCA.

\textbf{Second, we establish fundamental tradeoffs.} We extend previous work on Network Utility Maximization (NUM)~\cite{num-kelly,num-srikant,num-low,duality-vegas} by showing that contracts determine the four key metrics mentioned above. We prove these tradeoffs mathematically and identify exactly two corner points in the tradeoff space that represent optimal choices for specific objectives.

\textbf{Third, we provide actionable design and analysis blueprints.} We present an easy-to-follow workflow for CCA design and analysis that prevents common mistakes and reveals fundamental tradeoffs. For design: (1) pick a contract by choosing input/output, shape, and parameters; (2) implement dynamics to follow the contract. For analysis: (1) compute the CCA's contract; (2) locate it in the tradeoff space; (3) identify issues from shifts or clamps; (4) compare dynamics. Our blueprints are intuitive, aligning with how the community designs CCAs, and make tradeoffs obvious from contract choices.

The contracts framework reveals that any systematization helping designers navigate the CCA design space brings us closer to good CCAs for practical scenarios. By following our methodology, future research can avoid repeating common mistakes while making conscientious tradeoff decisions rather than inadvertent ones.


\section{Introduction}

Congestion control algorithms (CCAs) play a critical role in ensuring fair and efficient allocation of bandwidth in networks. Despite four decades of research asking fundamental questions—What is the best CCA? Do we need specialized CCAs or can we find one that fits many network scenarios? What are the fundamental limits of CCA performance?—the search for answers has remained elusive.

The challenge stems from CCAs operating in partially observable environments where they lack direct visibility into link capacities, network topology, or competing flows. To achieve fairness, CCAs must encode information about fair shares into observable network signals. For instance, Reno uses loss rate to coordinate fair shares, with each endpoint transmitting at an average rate $\propto 1/\sqrt{\text{loss rate}}$. We refer to such communication mechanisms as \emph{contracts}.

Traditionally, CCAs were designed to avoid congestion collapse, with fairness properties analyzed retrospectively~\cite{fairness-chiu-jain,num-srikant,num-low,num-kelly}. With the rise of applications like real-time communication and short remote-procedure calls (RPCs), newer CCA designs prioritized local performance metrics like latency and convergence time. However, this ``local'' perspective often led to undesirable fairness outcomes. For instance, TIMELY~\cite{timely} has been shown to have infinite fixed points, causing unfair rate allocations~\cite{ecn-vs-delay}.

\textbf{Contributions.} We contribute to this effort by building an abstraction of \emph{contracts} that formalizes the mechanisms CCAs use to coordinate fairness. This leads to five key contributions:

\textbf{(C1) Contract abstraction.} We formalize contracts as the communication mechanisms that CCAs use to encode fair shares into observable network signals (e.g., delay, loss, ECN). We show that the choice of contract—often made implicitly—fully determines four key metrics: \emph{robustness} to signal noise, \emph{fairness} in multi-bottleneck networks, amount of \emph{congestion}, and \emph{generality} (range of supported link rates).

\textbf{(C2) Fundamental tradeoffs.} We discover and analytically quantify previously unknown tradeoffs that apply to a broad class of CCAs. Robustness and fairness improve with gradual contracts, while congestion and generality improve with steeper contracts. We prove these tradeoffs mathematically and identify exactly two corner points representing optimal choices for specific objectives.

\textbf{(C3) Design mistakes and performance issues.} We identify previously unknown scenarios and avoidable design mistakes that cause severe performance degradation (near-zero throughput or starvation) in a wide range of CCAs, including BBR~\cite{bbr}, Vegas~\cite{vegas}, ICC~\cite{icc}, and Swift~\cite{swift}. Our methodology works for analytically designed CCAs, black-box implementations (e.g., Tao~\cite{tao,remy}), and learned CCAs (e.g., PCC~\cite{pcc}, Astraea~\cite{astraea}).

\textbf{(C4) Design and analysis blueprints.} We provide actionable workflows that make tradeoffs and mistakes intuitive. For design: (1) pick a contract (input/output, shape, parameters); (2) implement dynamics. For analysis: (1) compute the contract; (2) locate it in tradeoff space; (3) identify issues; (4) compare dynamics. This helps avoid performance mistakes and enables conscientious selection of Pareto-optimal tradeoffs.

\textbf{(C5) Empirical validation.} We validate our findings using simulation and emulation, achieving near-perfect match between analysis and measurements across the performance metrics and tradeoffs we identify.

The contracts framework reveals that any systematization helping designers navigate the CCA design space brings us closer to good CCAs for practical scenarios. By following our methodology, future research can avoid repeating common mistakes while making conscientious tradeoff decisions rather than inadvertent ones.


Congestion control algorithms (CCAs) play a critical role in ensuring fair and
efficient allocation of bandwidth in networks. Despite this, reasoning about
their fairness has been ad hoc. Traditionally, CCAs were designed to avoid
congestion collapse, with fairness properties analyzed
retrospectively~\cite{fairness-chiu-jain,num-srikant,num-low,num-kelly}. With
the rise of applications like real-time communication and short
remote-procedure calls (RPCs), newer CCA designs prioritized local
performance metrics like latency and convergence time. However, this local
perspective often led to undesirable fairness outcomes. For instance, 
TIMELY~\cite{timely} has infinite fixed points, causing unfair rate 
allocations~\cite{ecn-vs-delay}.

The search for a CCA that meets key efficiency, latency, fairness, and 
robustness objectives has been long and elusive. Real-world networks are 
complicated and hard to predict, and empirical and theoretical evidence 
suggests that all objectives are not simultaneously 
achievable~\cite{starvation, ccmatic, ecn-vs-delay, throughput-vs-fairness, 
faircloud,num-low-book}. Consequently, any CCA design must make difficult 
tradeoffs. Any systematization that helps designers navigate the CCA design 
space brings us closer to good CCAs for practical scenarios.

\myparagraph{Contributions} We contribute to this effort by (C1) building an
abstraction of \emph{contracts} that formalizes how CCAs coordinate fairness 
(\autoref{sec:motivation}, \autoref{sec:contracts}). This led us to (C2) 
discover and analytically quantify previously unknown tradeoffs across a broad 
class of CCAs (\autoref{sec:metrics-tradeoffs}), and (C3) identify previously 
unknown scenarios and avoidable design mistakes that cause severe performance 
degradation in CCAs including BBR~\cite{bbr}, Vegas~\cite{vegas}, 
ICC~\cite{icc}, and Swift~\cite{swift} (\autoref{sec:motivation}, 
\autoref{sec:pitfalls}). Our methodology works for both analytically designed 
CCAs and black-box implementations, \eg, Tao (Remy)~\cite{tao, remy} and 
learned CCAs like PCC~\cite{pcc} and Astraea~\cite{astraea}. Using contracts 
and our learnings, we (C4) build blueprints for CCA design and analysis that 
make tradeoffs and mistakes intuitive and actionable (\autoref{sec:motivation}). 
(C5) We validate our findings using simulation and emulation, finding 
near-perfect matches between analysis and measurements 
(\autoref{sec:empirical}).

\myparagraph{Contracts} CCAs operate in partially observable environments---they 
do not know network link rates, topology, routing, or competing flow counts. To 
achieve fairness, CCAs encode fair share information into observable network 
signals. For instance, Reno uses loss rate to coordinate fair shares, with each 
endpoint transmitting at an average rate $\propto 1/\sqrt{\texttt{loss rate}}$. 
We refer to such communication mechanisms as \emph{contracts}. All existing 
CCAs that share bandwidth fairly incorporate a contract, either implicitly 
(\eg, Reno~\cite{mathis-model}, Vegas~\cite{duality-vegas}) or explicitly 
(\eg, TFRC~\cite{tfrc}, Swift~\cite{swift}).

CCA contracts differ in the signals they use and their shape. Delay-based CCAs 
encode fair share as: ``$1/\texttt{delay}$'' \cite{vegas,fasttcp,copa}, 
``$1/\texttt{delay}^2$'' \cite{swift}, or ``$e^{-\texttt{delay}}$'' 
\cite{starvation}, where $\texttt{delay}$ is queuing delay (\eg $\rtt - \min 
\rtt$).\footnote{Throughout this paper, ``$\texttt{delay}$'' means queuing 
delay.} Contracts effectively parameterize the CCA design space without fully 
specifying dynamics. For instance, TCP-friendly 
CCAs~\cite{reno, newreno, tfrc, binomial-infocom} follow Reno's contract 
(\ie ensure rate $\propto 1/\sqrt{\texttt{loss rate}}$) but differ in 
stability and convergence properties.

\myparagraph{Tradeoffs} This variety raises the question: ``What are the 
tradeoffs between different contract choices?'' We discovered that contract 
choice fully determines four key metrics: (1) \emph{robustness} to noise in 
congestion signals, (2) \emph{fairness} in multi-bottleneck networks, 
(3) \emph{congestion} (\eg, delay, loss), and (4) \emph{generality} 
(\eg, supported link rate range). Robustness and fairness improve with gradual 
contracts, while congestion and generality improve with steeper contracts 
(\autoref{sec:metrics-tradeoffs}). Thus, we cannot optimize all four metrics 
simultaneously.

Similar tradeoffs have been explored before. \cite{starvation} discusses a 
special case where full generality precludes simultaneous robustness and 
bounded congestion variation. We find that their proposed workarounds cause 
unfairness (\autoref{sec:metrics-tradeoffs}, \autoref{sec:pitfalls}). 
\cite{ecn-vs-delay} shows delay-based CCAs cannot simultaneously ensure fixed 
delays and fairness. The NUM literature~\cite{num-kelly, num-srikant, num-low, 
duality-vegas} has studied subsets of these tradeoffs for individual CCAs. To 
our knowledge, we are the first to uncover and generalize these tradeoffs 
across many CCAs.

\myparagraph{Mistakes} We use contracts to identify avoidable design mistakes 
(\autoref{sec:motivation}, \autoref{sec:pitfalls}). CCAs with extreme contract 
shapes (\eg, logarithmic, exponential), shifts, clamps, or intercepts can 
starve flows---affecting BBR, ICC, and Astraea. Additionally, we show that 
AIMD on delay (used in SMaRTT~\cite{smartt}, STrack~\cite{strack}, and 
1RMA~\cite{1rma}) creates starvation in multi-bottleneck topologies due to 
fixed end-to-end thresholds. With explicit contracts, MIMD updates can achieve 
exponentially fast convergence while maintaining fairness, eliminating the 
need for AIMD in many cases.

\myparagraph{Blueprints} We argue that CCA design should start with contract 
selection. Contracts prevent mistakes better than other design patterns. Many 
methodologies start from utility functions---local utilities (\eg, 
``$\log(\texttt{tput}) - \log(\delay)$'' in Copa~\cite{copa}), global 
utilities (\eg, NUM/Remy~\cite{remy}), or RL reward functions~\cite{astraea}. 
These hide tradeoffs, creating illusions of unilateral optimization when 
metrics are fundamentally intertwined (\autoref{sec:metrics-tradeoffs}). 
Contracts force conscientious tradeoff choices and Pareto-optimal point selection. 
They are also more intuitive---tradeoffs are obvious from contract choice, 
aligning with how many CCAs are designed (\eg, Swift~\cite{swift}, 
TFRC~\cite{tfrc} start with target rate equations).

We discuss contract limitations and potential workarounds 
(\autoref{sec:limitations}, \autoref{sec:discussion}).



\section{Introduction}

End-to-end congestion control algorithms (CCAs) play a critical role in allocating bandwidth fairly and efficiently. Historically, CCAs were designed to prevent congestion collapse, and fairness properties were analyzed only in hindsight~\cite{fairness-chiu-jain,num-srikant,num-low,num-kelly}. More recent CCAs prioritize local performance metrics such as low latency and fast convergence to better serve modern workloads like real-time communication and short RPCs. However, these localized optimizations often come at the cost of fairness. For example, TIMELY~\cite{timely} admits infinitely many fixed points, leading to highly unfair allocations~\cite{ecn-vs-delay}.

Despite decades of research, designing a CCA that jointly achieves efficiency (generality), low congestion (latency), fairness, and robustness remains elusive. Empirical and theoretical results show that these goals are fundamentally in tension~\cite{starvation,ccmatic,ecn-vs-delay,throughput-vs-fairness,faircloud,num-low-book}. Thus, any CCA must make tradeoffs. A unifying framework that reveals and navigates these tradeoffs can guide better CCA design.

\vspace{1ex}
\noindent\textbf{Contributions.} We introduce \textit{contracts}, a unifying abstraction that formalizes how CCAs encode fair shares into observable signals (\S\ref{sec:motivation}, \S\ref{sec:contracts}). This abstraction allows us to:
\begin{itemize}
    \item[(C1)] Identify the implicit or explicit coordination mechanisms (contracts) used by CCAs to achieve fairness.
    \item[(C2)] Derive analytical tradeoffs between four key performance metrics: robustness to noise, fairness in multi-bottleneck topologies, congestion (delay/loss), and generality (supported link rate range) (\S\ref{sec:metrics-tradeoffs}).
    \item[(C3)] Use these tradeoffs to uncover avoidable design pitfalls—including starvation and instability—in a range of CCAs including BBR~\cite{bbr}, Vegas~\cite{vegas}, Swift~\cite{swift}, ICC~\cite{icc}, and learned CCAs such as PCC~\cite{pcc} and Astraea~\cite{astraea} (\S\ref{sec:motivation}, \S\ref{sec:pitfalls}).
    \item[(C4)] Provide a contract-first blueprint for designing and analyzing CCAs, enabling principled tradeoff selection and prevention of common mistakes (\S\ref{sec:motivation}).
    \item[(C5)] Empirically validate the tradeoffs and pitfalls through simulation and emulation, showing near-perfect alignment with analytical predictions (\S\ref{sec:empirical}).
\end{itemize}

\vspace{1ex}
\noindent\textbf{Why contracts?} CCAs operate in partially observable environments—they do not know link rates, routing, or the number of competing flows. To share bandwidth fairly, flows must implicitly agree on how to interpret shared signals (e.g., loss rate or delay). For instance, Reno converges to a rate proportional to $1/\sqrt{\texttt{loss rate}}$. We call such mappings \textit{contracts}.

Different CCAs use different contracts. Delay-based CCAs encode fair share as $1/\texttt{delay}$~\cite{vegas}, $1/\texttt{delay}^2$~\cite{swift}, or $e^{-\texttt{delay}}$~\cite{starvation}. Contracts parameterize the space of fair CCAs without fully defining their dynamics. For example, TCP-friendly CCAs such as Reno, NewReno, and TFRC~\cite{tfrc} follow Reno's contract but differ in stability and convergence time.

\vspace{1ex}
\noindent\textbf{Tradeoffs.} We find that a CCA’s contract fully determines four steady-state metrics: robustness, fairness, congestion, and generality. Gradual contracts (e.g., $1/\texttt{delay}$) improve robustness and fairness, while steeper contracts (e.g., $1/\texttt{delay}^2$) reduce congestion and expand generality. Therefore, no single contract can optimize all four metrics simultaneously.

This generalizes known results~\cite{starvation,ecn-vs-delay} and frames them in a broader context. For example, \cite{ecn-vs-delay} shows that delay-based CCAs cannot ensure fixed delay and fairness unless the contract is bijective. We go further to show that contract shape quantitatively determines tradeoffs and that these tradeoffs hold across many topologies and CCAs (\S\ref{sec:metrics-tradeoffs}).

\vspace{1ex}
\noindent\textbf{Avoiding design pitfalls.} Contracts provide a lens to identify common but avoidable mistakes:
\begin{itemize}
    \item \textit{Extreme contract shapes} (e.g., exponential, logarithmic) or shifts can lead to starvation. We observe this in BBR, ICC, and Astraea.
    \item \textit{Fixed delay thresholds at endpoints} (as in AIMD-on-delay used by SMaRTT, STrack, and 1RMA) cause starvation in multi-hop topologies. For example, a flow with larger RTT may always exceed the target delay and never increase its rate.
    \item \textit{Misuse of AIMD}: Even when a CCA has an explicit contract (e.g., Swift), using AIMD instead of MIMD results in slow convergence. Contracts make it possible to use stable MIMD dynamics for fast convergence.
\end{itemize}

\vspace{1ex}
\noindent\textbf{Design blueprint.} Contracts offer a natural starting point for both CCA design and analysis. Existing approaches often start from utility functions (e.g., NUM~\cite{num-kelly}, Copa~\cite{copa}, Remy~\cite{remy}, or RL-based reward functions~\cite{astraea}) and bury tradeoffs in obscure parameters. In contrast, contracts make tradeoffs transparent and actionable. They compel designers to explicitly reason about how fair shares are encoded in congestion signals.

We advocate a \textit{contract-first blueprint} where one first chooses the contract (signal, shape, scaling) and then implements dynamics to follow it. This blueprint leads to designs that are both performant and interpretable, and helps avoid the pitfalls we identify. Finally, we discuss limitations and possible extensions of the contracts framework, including inter-CCA fairness and dynamic contracts (\S\ref{sec:limitations}, \S\ref{sec:discussion}).



\myparagraph{Blueprints} We advocate for a contract-first approach to CCA design and analysis. Contracts offer a natural, intuitive foundation: they make tradeoffs between key performance metrics immediately apparent—often requiring little to no algebra—and align with how many CCAs are already designed. For instance, CCAs like Swift~\cite{swift} and TFRC~\cite{tfrc} begin with a target rate equation and build control dynamics around it.

Compared to alternative design patterns, contracts are better suited to avoid common pitfalls. Many existing methodologies instead start from a utility function—local (e.g., $\log(\texttt{tput}) - \log(\delay)$ in Copa~\cite{copa}), global (e.g., NUM/Remy~\cite{remy}), or learned reward functions in RL~\cite{astraea}). These approaches often obscure inherent tradeoffs, giving the false impression that latency or throughput can be optimized in isolation. In reality, these metrics are tightly coupled with fairness, robustness, and generality (\autoref{sec:metrics-tradeoffs}). As a result, many designs inadvertently commit to suboptimal tradeoff points due to unrelated design decisions (\autoref{sec:contracts}, \autoref{sec:metrics-tradeoffs}, \autoref{sec:pitfalls}).

Contracts, in contrast, compel the designer to explicitly confront these tradeoffs and make informed, conscientious choices. This enables deliberate selection of Pareto-optimal designs, rather than relying on accidental artifacts of other design components.


==> sections/archive/scratch.tex <==
\section{Conclusion}

We introduced contracts as a unifying framework for understanding congestion control algorithms, revealing fundamental tradeoffs between robustness, fairness, congestion, and generality. Our analysis shows that contract choice—often an implicit design decision—directly determines these key performance metrics, making simultaneous optimization impossible. 

We identified common design pitfalls that lead to starvation and poor performance, demonstrating how contract analysis can prevent these issues without implementation or measurement. Our empirical validation across diverse CCAs confirms that contract-based performance predictions closely match real behavior.

This work establishes a principled foundation for CCA design: contracts should be explicit, conscious choices driven by desired steady-state performance requirements, with dynamics designed separately for convergence properties. We hope this framework will guide future CCA development toward Pareto-optimal designs that make tradeoffs explicit rather than accidental.



\myparagraph{Implications for measurement} Measurement of workloads and network
environments can guide which metrics to prioritize in the tradeoff space. For
instance, assessing fairness requires understanding how often flows experience
multi-hop congestion and the typical number of flows or hops involved. Recent
work~\cite{stop-cca-fairness} suggests that such contention may be rare on the
Internet, implying that fairness may be less critical in some contexts. 

For robustness, it is important to quantify the magnitude and frequency of non-congestive delay and loss variations. On the workload side, network-level metrics may not align with application-level goals—for example, \cite{sudarsanan-ml-cc} shows that some AI collectives prefer unfair bandwidth allocations for better job performance.


\myparagraph{Implications for measurement} Contract tradeoffs highlight
critical measurement needs for CCA design. For fairness, we need data on
multi-hop congestion frequency and typical flow/hop counts—recent work suggests
flows rarely contend on the Internet~\cite{stop-cca-fairness}, potentially
de-prioritizing fairness. For robustness, we need measurements of
non-congestive delay and loss patterns. However, CCA designer metrics may not
align with application needs—AI collectives~\cite{sudarsanan-ml-cc} may
prioritize throughput over fairness or bounded delay.



In general, a CCA's contract depends on the network topology and competing
traffic; when this dependence is absent, computing the contract reduces to
simple program analysis without network assumptions.

\subsection{Computing contracts}
\label{sec:computing-contracts}

Contract functions can be obtained by analyzing a CCA's steady-state behavior on dumbbell and parking lot topologies. In general, contracts may depend on network parameters (capacity, RTprop, buffer sizes). When contracts are network-independent, computing them reduces to simple program analysis without network assumptions. When contracts depend on the network, analysis requires understanding CCA behavior across different network conditions.

This analysis can be done analytically (via fluid model analysis~\cite{ecn-vs-delay}) or empirically by collecting steady-state observations. For CCAs with limit-cycle equilibria (\eg, Reno/DCTCP sawtooth behavior), contracts describe cycles rather than fixed points, \eg, DCTCP's contract is ``$\texttt{critical\_cwnd} = 1/(\texttt{avg ECN marking rate})^2$''~\cite{dctcp}. Multi-modal CCAs like Copa require compound functions that switch between contracts based on detected flow types.

The literature provides contracts for most existing CCAs (see ``$\func(\s)$'' column in \autoref{tab:contracts-summary}), allowing us to focus on analyzing contract impact rather than derivation. We demonstrate both analytical and empirical approaches below.

\myparagraph{Analytical derivation (Vegas)} Vegas updates \cwnd based on $\texttt{diff} = \cwnd/\rtt - \cwnd/\texttt{RTprop}$ versus threshold $\alpha_{\rate}$. At steady-state, $\texttt{diff} = \alpha_{\rate}$, yielding Vegas's contract: $\rate = \alpha_{\rate} \cdotp \texttt{RTprop}/\delay$. This contract is network-independent after removing RTprop bias by setting $\alpha_{\rate} = \alpha_{\texttt{pkts}}/\texttt{RTprop}$~\cite{vegas-linux-2.2}.

\myparagraph{Black-box derivation (Astraea)} For reinforcement learning CCAs like Astraea~\cite{astraea}, we query the neural network's state-action mapping to find fixed points where action = 0 (no \cwnd change). Curve fitting these points yields the learned contract (\autoref{fig:astraea-fit}).

\myparagraph{Empirical validation (Pantheon CCAs)} We automatically derived contracts for all Pantheon~\cite{pantheon} CCAs using 60-second runs across varied network conditions (24-96 Mbps, 40ms RTprop, 2-8 flows). Of 15 functional CCAs, 7 proved unfair (different rates despite similar signals) and lack contracts (\autoref{fig:pantheon-unfair}), while 6 exhibit clear contracts (\autoref{tab:pantheon-contracts}). Network-dependent contract parameters (\eg, BBR's delay shift equals RTprop) require careful calibration for deployment.



\myparagraph{Computing contracts}
In principle, we can obtain the contract function of a CCA by running it on a diverse set of topologies (e.g., dumbbell and parking lot) with varying capacities, propagation delays, buffer sizes, and flow counts. By grouping steady-state observations that yield the same rate for a given aggregate statistic, we obtain equivalence classes that define the CCA’s contract.

This process can be done empirically or analytically (e.g., using fluid models~\cite{ecn-vs-delay}). In many cases, program analysis suffices without simulating a network; e.g., for Vegas, equilibrium behavior directly reveals the contract. For CCAs with limit-cycle rather than fixed-point equilibria, such as Reno or DCTCP, the contract describes behavior over a cycle—e.g., DCTCP's critical window: $\texttt{cwnd} = 1/(\texttt{avg ECN marking rate})^2$~\cite{dctcp}.

Importantly, it suffices to run a single flow while varying link capacity to determine the rate vs. congestion mapping. However, multi-modal CCAs (e.g., Copa) may switch modes depending on noise or competition. For instance, Copa emulates Reno when detecting loss-based flows~\cite{copa}. In such cases, the aggregate statistic may be multi-dimensional, and $\func$ may be a compound function. For clarity, we focus on homogeneous settings where flows use the same mode.

The literature has computed contracts for most CCAs; we cite these in the $\func(\s)$ column of~\autoref{tab:contracts-summary}. Our analysis assumes these results hold—e.g., Copa does not emulate Reno when competing with itself. Even for CCAs where fluid modeling is intractable, equilibrium behavior is generally well understood—e.g., BBR encodes fair share using delay~\cite{starvation} or growth in delivery rate~\cite{bbr-rate-contract} depending on mode.

\myparagraph{Analytical example (Vegas~\cite{num-srikant})}
Vegas updates \cwnd by comparing $\texttt{diff} = \cwnd/\rtt - \cwnd/\texttt{RTprop}$ to $\alpha_{\rate}$. It increases or decreases \cwnd based on whether diff exceeds $\alpha_{\rate}$. At equilibrium, $\texttt{diff} = \alpha_{\rate}$, which gives:
\[
\rate = \alpha_{\rate} \cdot \texttt{RTprop} / \delay
\]
This contract exhibits RTprop bias. Implementations remove this by scaling $\alpha_{\rate} = \alpha_{\texttt{pkts}}/\texttt{RTprop}$~\cite{vegas-linux-2.2}. Reno’s RTT bias can similarly be removed via TFRC~\cite{tfrc}.

\myparagraph{Analytical example (Astraea~\cite{astraea})}
Astraea is an RL-based CCA that implicitly learns a contract. We query its neural network for actions across a range of delay and capacity inputs. Actions $>1$ increase \cwnd, $<1$ decrease, and $=0$ implies fixed point. Each link capacity corresponds to a unique delay with action zero. Fitting a curve of the form $\rate = a(\delay + b)^c + d$ gives Astraea's contract (\autoref{fig:astraea-fit}).

\myparagraph{Empirical contracts (Pantheon CCAs)}
We empirically derive contracts for CCAs in Pantheon~\cite{pantheon}. We run each CCA on a dumbbell topology (60s duration, link capacities 24/48/96 Mbps, 40 ms RTprop, 4 BDP buffer) with 2–8 flows (1 BDP for Cubic). For each run, we collect throughput and three statistics (avg delay, p50 delay, loss rate) and fit curves $\rate = \func(\s)$ that minimize MSE.

Of 17 CCAs, we omit QUIC Cubic and Verus due to software issues. Of the remaining 15, two (SCReAM, WebRTC) show $\approx 0$ throughput, and seven (Indigo, Fillp/FillpSheep, PCC variants, TaoVA) are unfair—i.e., same statistic yields different rates across flows—indicating no contract (\autoref{fig:pantheon-unfair}). The remaining six yield the contracts in \autoref{tab:pantheon-contracts}.

These empirical contracts are valid within the tested network range. Some CCAs (e.g., PCC-Vivace) appear fair only at high capacity (e.g., 96 Mbps), with contracts like $\rate \propto \texttt{avg delay}^{-0.4}$. Delay shifts (e.g., 46.91 ms in BBR) vary with RTprop or buffer size. Some CCAs may also use nonstandard statistics or multi-modal mappings, requiring more extensive experimentation to fully capture.




\subsection{Computing contracts}
\label{sec:computing-contracts}

Contract functions can be obtained by analyzing a CCA's steady-state behavior on dumbbell and parking lot topologies. This analysis can be done analytically (via fluid model analysis~\cite{ecn-vs-delay}) or empirically by collecting steady-state observations across different network conditions and building equivalence classes based on aggregate statistics.

For most CCAs, this reduces to simple program analysis without network simulation. For CCAs with limit-cycle equilibria (\eg, Reno/DCTCP sawtooth behavior), contracts describe cycles rather than fixed points, \eg, DCTCP's contract is ``$\texttt{critical\_cwnd} = 1/(\texttt{avg ECN marking rate})^2$''~\cite{dctcp}. Multi-modal CCAs like Copa require compound functions that switch between contracts based on detected flow types.

The literature provides contracts for most existing CCAs (see ``$\func(\s)$'' column in \autoref{tab:contracts-summary}), allowing us to focus on analyzing contract impact rather than derivation. We demonstrate both analytical and empirical approaches below.

\myparagraph{Analytical derivation (Vegas)} Vegas updates \cwnd based on $\texttt{diff} = \cwnd/\rtt - \cwnd/\texttt{RTprop}$ versus threshold $\alpha_{\rate}$. At steady-state, $\texttt{diff} = \alpha_{\rate}$, yielding Vegas's contract: $\rate = \alpha_{\rate} \cdotp \texttt{RTprop}/\delay$. This RTprop bias is easily removed by setting $\alpha_{\rate} = \alpha_{\texttt{pkts}}/\texttt{RTprop}$~\cite{vegas-linux-2.2}.

\myparagraph{Black-box derivation (Astraea)} For reinforcement learning CCAs like Astraea~\cite{astraea}, we query the neural network's state-action mapping to find fixed points where action = 0 (no \cwnd change). Curve fitting these points yields the learned contract (\autoref{fig:astraea-fit}).

\myparagraph{Empirical validation (Pantheon CCAs)} We automatically derived contracts for all Pantheon~\cite{pantheon} CCAs using 60-second runs across varied network conditions (24-96 Mbps, 40ms RTprop, 2-8 flows). Of 15 functional CCAs, 7 proved unfair (different rates despite similar signals) and lack contracts (\autoref{fig:pantheon-unfair}), while 6 exhibit clear contracts (\autoref{tab:pantheon-contracts}). Contract parameters depend on network conditions (\eg, BBR's delay shift equals RTprop), requiring careful calibration for deployment.





On dumbbell topologies, AIMD on delay functions correctly, inducing a Reno-like contract $\x = 1/\sqrt{\s}$ where \s represents high-delay probability (inverse of bytes between high-delay events) rather than loss probability. However, it causes starvation due to fixed delay thresholds. All hosts attempt to maintain delay around the same target value, but flows observing delays from different hop combinations cannot simultaneously achieve the same delay target.

\autoref{fig:starvation-aimd-delay} demonstrates this failure in a 2-hop parking lot. Short flows (\f[1], \f[2]) oscillate between the delay threshold and half-threshold (\textcolor{TextGray}{gray}), while the long flow (\f[0]) observes their sum—always exceeding the threshold. Consequently, \f[0] never increments \cwnd and starves.


On dumbbell topologies, AIMD on delay functions correctly, inducing a Reno-like contract $\x = 1/\sqrt{\s}$ where \s represents high-delay probability (inverse of bytes between high-delay events) rather than loss probability. However, it causes starvation in multi-bottleneck scenarios due to fixed delay thresholds. All hosts attempt to maintain delay around the same target value, but with multiple bottlenecks, flows observing delays from different hop combinations cannot simultaneously achieve the same delay target.

\autoref{fig:starvation-aimd-delay} demonstrates this failure in a 2-hop parking lot. Short flows (\f[1], \f[2]) oscillate between the delay threshold and half-threshold (\textcolor{TextGray}{gray}), while the long flow (\f[0]) observes their sum—always exceeding the threshold. Consequently, \f[0] never increments \cwnd and starves.


Unlike the robustness issue in \cite{starvation}, this problem is not fundamental and is easily avoided by removing X-intercepts (e.g., $\rate = 1/\delay$). The \cite{starvation} issue stems from Y-axis asymptotes where high fair shares (>100 Mbps) map to near-zero delays (\autoref{fig:error-shift} left). This asymptote is fundamentally unavoidable when supporting arbitrarily large rates with monotonically decreasing contracts, though transmission delays naturally provide a lower bound since they scale as $1/\bw$ with decreasing capacity.


Unlike the robustness issue in \cite{starvation}, this problem is not fundamental and is easily avoided by removing X-intercepts (e.g., $\rate = 1/\delay$). The \cite{starvation} issue stems from Y-axis asymptotes where high fair shares (>100 Mbps) map to near-zero delays (\autoref{fig:error-shift} left). This asymptote is fundamentally unavoidable when supporting arbitrarily large rates with monotonically decreasing contracts. While X-intercepts may seem appealing for bounding delays, they are unnecessary since transmission delays naturally scale as $1/\bw$ with decreasing capacity, providing an inherent lower bound.

Unlike the robustness issue in \cite{starvation}, this problem is not fundamental and is easily avoided by removing X-intercepts (e.g., $\rate = 1/\delay$). The \cite{starvation} issue stems from Y-axis asymptotes where high fair shares (>100 Mbps) map to near-zero delays (\autoref{fig:error-shift} left). This asymptote is fundamentally unavoidable when supporting arbitrarily large rates with monotonically decreasing contracts. While X-intercepts may seem appealing for upper-bounding delays by a constant, this is worthless since transmission delays—which scale as $1/\bw$ with decreasing capacity—provide a variable lower bound that will eventually exceed any fixed constant.


\myparagraph{Avoid shifting contracts} CCAs like Swift~\cite{swift} define target delay ($\rtt - \min \rtt$) as $\texttt{target\_delay} = b + 1/\rate$. While setting positive $b$ to maintain minimum delay for high utilization may seem convenient, shifting contracts causes severe unfairness (\autoref{fig:error-shift} right). We demonstrate empirical unfairness in BBR due to contract shifts in \autoref{sec:empirical}. Instead, use scaling (\autoref{sec:metrics-tradeoffs}) to maintain minimum delay.

Since target delay is the contract's inverse and its integral defines the CCA's utility function (\autoref{sec:contracts}), shifts alter utility and rate allocations. For contract $\x = \func(\s) = 1/(\s-b)$, the parking lot throughput ratio becomes $\max_{\bw} \frac{\func(\s[k])}{\func(k\s[k])} = \frac{k\s[k] - b}{\s[k] - b}$. When $\s[k] = b + \epsilon$, this ratio approaches infinity as $\epsilon \to 0$, causing starvation.

Note that with RED-based ECN marking~\cite{red, ecn}, queue buildup can be shifted without altering steady-state ECN marking probability by adjusting RED parameters $K_{min}, K_{max}$—this changes queue size but preserves marking probability.


\myparagraph{Avoid extreme shape and intercepts} Astraea's linear contract and ICC's logarithmic contract exhibit poor robustness and fairness due to extreme shapes and X-intercepts. The fundamental issue is that low fair shares (e.g., 0.1-1 Mbps) map to delays clustered near the X-intercept (e.g., 40 ms) (\autoref{fig:error-shift} middle). Minor delay jitter thus creates large fair share estimation errors. In parking lot topologies (\autoref{fig:parking_lot}), when hop delays approach the X-intercept, the long flow (\f[0]) observes their sum, which exceeds the intercept delay. Attempting to reduce this "excessive" delay, \f[0] reduces its rate to zero and starves.

\autoref{fig:extreme-contract-bad} demonstrates these issues empirically: ambient emulation noise causes Astraea to starve flows at low fair shares (4 flows, 10 Mbps dumbbell, 30 ms RTprop, infinite buffer), while ICC starves the long flow in parking lot scenarios (3 flows, 2 hops, same parameters).

This robustness issue differs fundamentally from that in \cite{starvation}. Here, the problem stems from X-intercepts and is easily avoided (e.g., using $\rate = 1/\delay$). The \cite{starvation} issue involves Y-axis asymptotes where high fair shares (>100 Mbps) map to near-zero delays (\autoref{fig:error-shift} left)—a fundamental limitation when supporting arbitrarily large rates with monotonically decreasing contracts.

Crucially, contract analysis reveals these performance issues without running CCAs or understanding their internal mechanisms.


\myparagraph{Avoid extreme contracts and intercepts} Extreme contract shapes cause severe performance issues. Astraea's linear contract and ICC's logarithmic contract exhibit poor fairness and robustness due to X-intercepts and steep slopes (\autoref{fig:extreme-contract-bad}). Under modest conditions (10 Mbps capacity, 30 ms RTprop, infinite buffer), Astraea starves flows in 4-flow dumbbell topologies when delays approach its X-intercept, while ICC starves the long flow (\f[0]) in 3-flow parking lot topologies.




Contract analysis reveals these failures before empirical testing—the mathematical form immediately indicates where CCAs will break, regardless of their internal mechanisms. The root cause is that low fair shares map to delays near the X-intercept (\autoref{fig:error-shift} middle), making minor noise create large fair share discrepancies. This is avoidable by eliminating X-intercepts (e.g., Vegas's contract $1/\s$). This differs from the fundamental high-bandwidth issue where fair shares map to near-zero delays due to Y-axis asymptotes (\autoref{fig:error-shift} left)—a fundamental limitation that cannot be avoided.

\section{Learnings from contracts}
\label{sec:pitfalls}

\myparagraph{Avoid extreme contracts and intercepts} Extreme contract shapes and X-intercepts cause severe performance degradation. Astraea's linear contract and ICC's logarithmic contract both exhibit poor fairness and robustness (\autoref{fig:extreme-contract-bad}). Astraea starves flows when fair shares are low (delay approaches the contract's X-intercept), while ICC starves the long flow (\f[0]) in parking lot topologies. These failures occur under modest conditions: 10 Mbps capacity, 30 ms RTprop, infinite buffer, with Astraea tested on 4-flow dumbbell and ICC on 3-flow parking lot (2 hops).

Crucially, contract analysis reveals these performance issues before empirical testing. The contract shape immediately indicates failure modes—we need not understand the CCA's internal mechanisms to predict when and why it will break.


We quantify unfairness as the (worst-case) throughput ratio of $\f[k]$ to $\f[0]$. In steady-state, at each hop, the sum of the incoming rates equals the link capacity: $\forall i \in \{1, \ldots, k\}: \x[0] + \x[i] = \bw$, and each flow's rate follows the contract: $\forall i \in \{0, 1, \ldots, k\}: \x[i] = \func(\s[i])$. Say flow $\f[i]$'s sending rate is $\x[i]$, and it observes statistic $\s[i]$.

Function \agg describes how statistic \s accumulates across hops through $s_0 = \agg(s_1, s_2, \ldots, s_k)$—that is, what statistic $\f[0]$ observes when other flows see $s_1, s_2, \ldots, s_k$. For delays, $s_0 = \sum_{i=1}^{k} s_i$ since delays are additive. For loss and ECN marking rates, $s_0 = 1 - \prod_{i=1}^k (1-s_i)$ since survival probabilities multiply across hops. When loss rates (or ECN marking rates) are small (e.g., $10^{-2}$), \agg can be approximated as summation. For max per-hop delay (e.g., Poseidon~\cite{poseidon}), $s_0 = \max(s_1, s_2, \ldots, s_k)$.


The choice of contract fundamentally constrains CCA performance metrics. Conversely, specifying a desired metric value constrains the feasible contract choices, which in turn limits other metrics—creating fundamental tradeoffs.

We proceed by first defining key performance metrics and expressing their values in terms of the contract function \func. We then derive quantitative tradeoffs, showing how constraining one metric bounds the achievable values of others. Our metric definitions are unit-less to minimize dependence on network parameters (e.g., link capacity, RTprop).

Throughout this analysis, we use Vegas~\cite{vegas,duality-vegas} and Swift~\cite{swift} as running examples, with contracts $\x = 1/\s$ and $\x = 1/\s^2$ respectively, where \s represents delay. For clarity, we omit scaling constants that ensure dimensional consistency—in practice, the constants in Vegas's and Swift's contracts have units of bytes and byte-seconds respectively, yielding rates in bytes/second. \autoref{tab:contracts-summary} positions existing CCAs within the resulting tradeoff space.


\myparagraph{Empirical contract derivation (CCAs in Pantheon)} 
To demonstrate that (1) contracts are easily computable and (2) fair CCAs possess identifiable contracts, we empirically derive contracts for all CCAs in Pantheon~\cite{pantheon} using an automated procedure. We evaluate each CCA for 60 seconds on a dumbbell topology with link capacities of 24, 48, and 96 Mbps, 40 ms RTprop, 4 BDP buffer, and flow counts varying from 2 to 8 (except Cubic, which uses 1 BDP buffer). This yields throughput samples and three aggregate statistics: p50 delay, average delay, and loss rate. We derive contracts by fitting curves to these data points (\autoref{fig:pantheon-fit}) and selecting the statistic $\s$ and functional form that minimizes mean squared error.

Of the 17 CCAs available in Pantheon at the time of writing, we encountered deprecation/dependency issues with QUIC Cubic and Verus, leaving 15 testable CCAs. Our analysis reveals three categories: (1) 2 CCAs (SCReAM and WebRTC) achieve near-zero utilization (consistent with prior Pantheon reports~\cite{scream-webrtc}), (2) 7 CCAs (Indigo, Fillp/FillpSheep, PCC-Allegro/Vivace/Experimental, TaoVA) exhibit unfairness (\autoref{fig:pantheon-unfair}), and (3) 6 CCAs demonstrate clear contracts.

Unfair CCAs produce different flow rates despite observing similar congestion signals, indicating the absence of a unique signal-to-rate mapping (contract function). However, these CCAs may exhibit fairness—and hence contracts—within narrower operational ranges. For example, PCC-Vivace and PCC-Experimental follow contracts $\texttt{avg delay}^{-0.4}$ and $\texttt{p50 delay}^{-0.46}$, respectively, when constrained to the 96 Mbps link scenario.

\autoref{tab:pantheon-contracts} presents the derived contracts for the 6 fair CCAs. Several caveats apply to our empirical approach: (1) contract validity is limited to our experimental network range, (2) delay shifts (e.g., 46.91 ms in BBR, 102 ms in LEDBAT) depend on specific network parameters like RTprop and buffer sizes—for BBR, the shift equals RTprop, and (3) CCAs may employ complex, compound contracts that vary across network conditions or utilize statistics beyond our three measured quantities. Comprehensive characterization would require broader experimental coverage.


While the philosophy of contracts shares mathematical foundations with Network
Utility Maximization (NUM)~\cite{num-kelly, num-srikant, num-low,
duality-vegas}, our framework provides novel insights and practical guidance
that extend beyond existing theory. Despite the established mathematical
underpinnings, many CCA designs—including recent proposals—continue to commit
easily avoidable mistakes that result in poor performance.

Beyond the well-documented issue of missing contracts (Mistake \#1), our
contracts framework has enabled us to identify several previously undocumented
design pitfalls detailed in Section~\ref{sec:pitfalls}. These discoveries
demonstrate that while the theoretical foundations exist, the practical
implications for algorithm design have not been adequately explored or
communicated. Our contracts lens makes these subtle but critical mistakes
sufficiently obvious to both identify in existing work and systematically avoid
in future designs.

\myparagraph{Methodology} We use htsim~\cite{htsim} for simulations (previously
used in MPTCP~\cite{mptcp}, NDP~\cite{ndp}, EQDS~\cite{eqds}) and
mahimahi~\cite{mahimahi}/Pantheon~\cite{pantheon}/mininet~\cite{mininet} for
emulation. We provide oracular RTprop access to all CCAs for two reasons: (1)
consistency across algorithms, as some like Swift target data-center
deployments where RTprop is known, and (2) to isolate fundamental
contract-based tradeoffs from RTprop estimation artifacts—Vegas performs poorly
due to misestimating RTprop since it doesn't explicitly drain queues like Copa
and BBR do. Since we validate negative results, these simplifications
strengthen our validation: if tradeoffs exist with oracular RTprop knowledge,
real-world performance will be worse due to estimation errors (under-estimation
causes under-utilization, over-estimation increases congestion).


\myparagraph{Methodology} We use htsim~\cite{htsim} for simulations (previously
used in MPTCP~\cite{mptcp}, NDP~\cite{ndp}, EQDS~\cite{eqds}) and
mahimahi~\cite{mahimahi}/Pantheon~\cite{pantheon}/mininet~\cite{mininet} for
emulation. We provide oracular RTprop knowledge to all CCAs for consistency
(appropriate for data-center deployments like Swift) and to isolate
contract-based tradeoffs from RTprop estimation artifacts. Since we validate
negative results, these simplifications strengthen our conclusions—if tradeoffs
exist with oracular information, real-world performance can only be worse due
to estimation errors.


\section{Limitations and Future Work}
\label{sec:limitations}

Our contracts framework represents a balance between expressivity and mathematical tractability. While this approach enables concrete analytical results, it necessarily imposes certain limitations that suggest directions for future research.

\subsection{Current Framework Limitations}

\myparagraph{Scope of Analysis}
Our contract definition focuses on steady-state behavior when CCAs compete with themselves, which limits our ability to directly reason about inter-CCA interactions. This restriction stems from our design choice to prioritize mathematical tractability over maximum expressivity—a tradeoff that enables the concrete performance bounds and design guidance presented in this work.

\myparagraph{Inter-CCA Fairness Complexities}
Real deployments often involve heterogeneous CCA interactions that our current framework cannot fully capture. For example:

\begin{itemize}
\item \textbf{Mode-switching algorithms:} Copa employs a delay-based contract when competing with itself but switches to emulating Reno upon detecting loss-based flows
\item \textbf{Implicit contract equivalence:} Vegas and Reno may achieve fairness despite different contracts when network conditions create equivalent mappings—for instance, RED-based packet drops can establish a relationship between queuing delay and loss rates that aligns their effective fair shares~\cite{num-low}
\item \textbf{Heuristic coexistence mechanisms:} BBR attempts TCP-friendliness by leaving "headroom" for loss-based CCAs, but this approach lacks the principled foundation that explicit contract adherence would provide
\end{itemize}

\myparagraph{Theoretical Completeness}
We have not yet established whether contracts (as currently defined) are necessary or sufficient for fairness. Resolving these theoretical questions would provide stronger design guidance and help determine whether contract-based approaches can fully characterize fair resource allocation.

\subsection{Future Research Directions}

\myparagraph{Expanding Framework Expressivity}
We plan to extend our contracts framework to address current limitations:

\begin{itemize}
\item \textbf{Multi-CCA environments:} Developing contract definitions that can reason about heterogeneous algorithm interactions
\item \textbf{Theoretical foundations:} Establishing necessity and sufficiency conditions for contract-based fairness
\item \textbf{Formal methods integration:} Drawing from contract-synthesis approaches in distributed systems~\cite{contract-synthesis}, which use $\omega$-regular grammars to describe behavioral traces, may provide tools for more expressive contract definitions
\end{itemize}

\myparagraph{Broadening Application Scope}
Our current blueprint primarily addresses steady-state long-flow scenarios. Key extensions include:

\begin{itemize}
\item \textbf{Transient behavior:} Incorporating short flows, incast scenarios, and other time-sensitive patterns that depend heavily on slow-start and initialization mechanisms
\item \textbf{Alternative control paradigms:} Extending analysis to receiver-based and credit-based control schemes
\item \textbf{Emerging metrics:} Adapting the framework to handle new performance objectives as application requirements evolve
\end{itemize}

We envision developing our design guidance into a living repository that evolves with the field's understanding of congestion control requirements.

\myparagraph{Practical Applications Beyond Design}
The contracts-first approach has potential applications beyond algorithm development:

\begin{itemize}
\item \textbf{Network measurement:} Improving reverse-engineering and classification of deployed CCAs~\cite{inspector-gadget, abagnale, ccanalyzer, nebby} by focusing on contract identification rather than implementation details
\item \textbf{Performance debugging:} Using contract analysis to diagnose unexpected behavior in production networks
\item \textbf{Standardization:} Providing a principled framework for evaluating and comparing CCA proposals in standardization contexts
\end{itemize}

These extensions would strengthen the practical impact of contracts-based congestion control analysis while maintaining the mathematical rigor that makes the framework useful for algorithm designers.



\subsection{Avoiding the mistakes using our blueprint of CCA design/analysis}
Unlike previous approaches, our contract-based methodology provides a systematic framework for CCA design that helps avoid common pitfalls. While no methodology can prevent all possible mistakes, following our blueprint significantly reduces the risk of design flaws that have plagued many CCAs.
Contracts offer advantages over existing methodologies in several key ways. In contrast to Network Utility Maximization (NUM), contracts provide a more intuitive and actionable approach that aligns with current CCA design practices. Many modern CCAs, such as Swift~\cite{swift} and TFRC~\cite{tfrc}, already implicitly start with a target rate equation and build dynamics around it.
Other methodologies—whether using local utilities (e.g., log-throughput minus log-delay in Copa), global utilities in NUM/Remy, or reward functions in RL—often obscure fundamental tradeoffs. These approaches create the illusion that metrics like latency can be optimized independently of other considerations, potentially leading to sub-optimal designs where tradeoffs emerge as unintended consequences of design decisions. In contrast, contracts explicitly surface these tradeoffs at the outset, forcing designers to make conscientious, informed choices.
We advocate that CCA design should begin with the selection of a contract. This approach requires designers to deliberately reason about how fairness coordination (fair shares) couples with congestion, and how this coupling affects steady-state performance metrics. Our framework provides comprehensive guidance through this process:
\begin{itemize}
\item We define contracts as a function (\autoref{sec:contracts})
\item We offer guidance on selecting shape/scale or derivative (\autoref{sec:metrics-tradeoffs})
\item We explain the implications of shifts in the contract (\autoref{sec:pitfalls})
\item We discuss input/output considerations (\autoref{sec:workarounds})
\item We show how to implement dynamics to follow a contract (\autoref{sec:canonical})
\end{itemize}
The tradeoffs we identify are fundamental to end-to-end CCAs, as some form of agreement between flows is necessary (as illustrated in \autoref{fig:assumptions-other-flows}). The only viable approach to circumvent these tradeoffs is to alter the input/output relationship within the contract to decouple performance metrics (\autoref{sec:workarounds}).
Beyond such input/output modifications, we contend that efforts to improve steady-state performance in end-to-end congestion control will likely rediscover CCAs already encompassed by our design space in \autoref{sec:metrics-tradeoffs}. This suggests that the contract-based approach offers a comprehensive framework that captures the essential design dimensions of congestion control.
For analyzing existing CCAs, we recommend a three-step process:
\begin{enumerate}
\item Compute the CCA's contract (\autoref{sec:compute})
\item Determine where this contract fits in the tradeoff space (\autoref{sec:metrics-tradeoffs})
\item Compare its dynamics with our canonical implementations (\autoref{sec:canonical})
\end{enumerate}


\subsection{A Blueprint for Principled CCA Design}

Despite decades of research, congestion control algorithm design remains prone to recurring patterns of mistakes. While no framework can prevent all possible errors, we propose a contracts-based design approach that systematically addresses the most common pitfalls.

\myparagraph{Why Contracts Over Other Frameworks}
The contracts framework offers distinct advantages over alternative design methodologies:

\begin{itemize}
\item Unlike Network Utility Maximization (NUM) models, contracts are intuitive and directly actionable, aligning with how practitioners actually develop CCAs (e.g., Swift~\cite{swift}, TFRC~\cite{tfrc} both begin with target rate equations)
\item Alternative approaches—whether based on local utilities (e.g., Copa's log(throughput) - log(delay)), global utilities (NUM/Remy), or RL reward functions—often obscure fundamental tradeoffs, creating an illusion that metrics like latency can be optimized independently
\item Contracts force designers to confront unavoidable tradeoffs explicitly at the outset, rather than discovering them as unintended consequences of implementation choices
\end{itemize}

\myparagraph{The Contracts-Based Design Process}
We propose a systematic approach to CCA design:

\begin{enumerate}
\item \textbf{Select a contract} (Section~\ref{sec:contracts}): Begin by defining the mathematical relationship between congestion signals and transmission rates
\item \textbf{Configure contract parameters} based on desired performance characteristics:
  \begin{itemize}
  \item Shape/scale (Section~\ref{sec:metrics-tradeoffs}): Determines fundamental tradeoffs between robustness, fairness, congestion, and generality
  \item Shift considerations (Section~\ref{sec:pitfalls}): Affects fairness properties
  \item Input/output selection (Section~\ref{sec:workarounds}): May enable working around certain tradeoffs
  \end{itemize}
\item \textbf{Implement appropriate dynamics} (Section~\ref{sec:canonical}): Choose update mechanisms that efficiently achieve the contract's steady-state behavior
\end{enumerate}

This process ensures that design decisions are made deliberately rather than accidentally, with full awareness of their performance implications.

\myparagraph{Analyzing Existing CCAs}
For analyzing existing algorithms, we recommend:
\begin{enumerate}
\item Compute the algorithm's contract (Section~\ref{sec:compute})
\item Position this contract within the tradeoff space (Section~\ref{sec:metrics-tradeoffs})
\item Evaluate its dynamics against optimal approaches (Section~\ref{sec:canonical})
\end{enumerate}

\myparagraph{Fundamental Limitations}
We believe the tradeoffs identified in this paper are fundamental to end-to-end congestion control, as they arise from the necessity of inter-flow agreement illustrated in Figure~\ref{fig:assumptions-other-flows}. Outside of changing the contract's input/output relationship (Section~\ref{sec:workarounds}), efforts to simultaneously optimize all performance metrics are likely to be futile—they will simply reinvent existing points in the design space covered in Section~\ref{sec:metrics-tradeoffs}. This insight should help focus future research on promising directions rather than rediscovering known tradeoffs.


\subsection{Tradeoff Summary and Contract Selection}

\myparagraph{Key Tradeoffs} 
Our analysis reveals fundamental tensions between performance metrics: robustness and fairness improve with more gradual contracts, while congestion management and generality benefit from steeper contracts. In Appendix~\ref{app:tradeoffs}, we mathematically prove these tradeoffs by examining each pair of competing metrics. For example, if we require an error factor $\leq \ef$ for noise level \ds, then congestion growth $\grow(n)$ must be at least $\Omega\left(\ds\frac{\log(n)}{\log(\ef)}\right)$. Importantly, these bounds are tight—we identify contracts (and consequently CCAs) that achieve them.

The nature of these tradeoffs depends critically on the aggregation function \agg. For $\agg = \sum$ (applicable to delay, loss rate, and ECN marking rate), the tradeoffs are unavoidable. However, for $\agg \in \{\max, \min\}$ (as with max per-hop delay in Poseidon~\cite{poseidon}), fairness can be independently achieved, leaving only the tradeoff between robustness versus congestion and generality.

\myparagraph{Corner Points in the Tradeoff Space}
Our analysis identifies two significant corner points that represent optimal choices under different priorities:

\begin{itemize}
\item \textbf{When prioritizing robustness:} The Exponential CCA from~\cite{starvation} provides optimal generality and congestion growth but exhibits poor fairness (Table~\ref{tab:contracts-summary}).
\item \textbf{When prioritizing fairness:} For proportional fairness ($\alpha=1$), Vegas delivers the best generality and congestion growth (with $\agg = \sum$). More generally, for $\alpha$-fairness, the contract $\func(\s) = \frac{1}{\sqrt[\alpha]{\s}}$ optimizes generality and congestion growth.
\end{itemize}

\subsection{Practical Contract Selection and Tuning}

The process of selecting and tuning a contract involves two distinct steps with different implications:

\begin{itemize}
\item \textbf{Shape selection} fixes the asymptotic behavior and fundamental tradeoffs
\item \textbf{Scale selection} determines constant factors and operational characteristics
\end{itemize}

\myparagraph{Selecting Contract Shape}
Unless employing tradeoff workarounds (Section~\ref{sec:workarounds})—which typically require in-network support or more fundamental congestion control research—practical deployments must choose between encoding information in delay, loss rate, or ECN marking rate. This choice should consider buffer sizes, ECN support, and dynamics (Section~\ref{sec:canonical}).

After selecting the signal type, designers must decide which corner point in the tradeoff space best suits their requirements. This decision fixes the contract shape (e.g., $\rate = 1/\s$ or $\rate = e^{-\s}$), establishing the fundamental performance characteristics of the algorithm.

\myparagraph{Tuning Contract Scale}
With the shape selected, designers must tune constant parameters to achieve specific operational goals. Importantly, these parameters involve inherent tradeoffs—optimizing for one metric necessarily constrains others:

\begin{itemize}
\item \textbf{For the exponential contract} ($\rate = \bw[0] e ^{-\s/\Sig[0]}$):
  \begin{itemize}
  \item Setting $\bw[0]$ establishes the maximum achievable rate, with any higher link capacity resulting in underutilization
  \item Setting $\Sig[0]$ controls robustness to noise (error factor = $e^{\ds/\Sig[0]}$), but simultaneously determines the delay range for a given capacity range
  \item If you prioritize robustness by increasing $\Sig[0]$, you necessarily increase delay for the same throughput
  \end{itemize}

\item \textbf{For the $\alpha$-fair contract} ($\rate = \bw[0] {\Sig[0]}^{\alpha} / \s^{\alpha}$):
  \begin{itemize}
  \item Setting $\bw[0]$ and $\Sig[0]$ together establishes the operating point where delay $\Sig[0]$ corresponds to rate $\bw[0]$
  \item For data centers with known maximum capacity $\Cmax$, setting minimum delay $\Smin$ (to ensure utilization or bound error factor by $1 + \ds/\Smin$) yields $\rate = \Cmax\Smin/\delay$
  \item If you prioritize supporting high link rates, you necessarily sacrifice bounded error factors as $\Smin$ approaches zero
  \end{itemize}
\end{itemize}

This fundamental distinction highlights the core tradeoff identified in~\cite{starvation}: exponential contracts ensure finite error factors but cannot support arbitrarily high capacities, while $\alpha$-fair contracts support unlimited capacities but cannot bound error factors.



\subsection{Motivation and Contribution}

While the philosophy of contracts shares mathematical foundations with Network Utility Maximization (NUM)~\cite{num-kelly, num-srikant, num-low, duality-vegas}, our framing offers several distinct advantages. We believe contracts provide a more intuitive and actionable framework that aligns with contemporary CCA design practices, where designers typically begin with a target rate equation and build dynamics around it.

Our work addresses a concerning pattern: despite the mathematical foundations being well-established, many CCA designs—including recent proposals—continue to commit avoidable mistakes that lead to suboptimal performance. These errors typically stem from:

\begin{itemize}
\item Myopically optimizing individual performance metrics (e.g., minimizing latency) without understanding their inherent coupling with other metrics like fairness
\item Treating congestion control purely as reaction to congestion signals without analytically reasoning about steady-state consequences
\item Failing to recognize how implementation details fundamentally alter the underlying contract and resulting performance characteristics \end{itemize}

We argue that effective CCA design should begin by explicitly selecting an appropriate contract, guided by the metrics and tradeoffs described in Section~\ref{sec:metrics-tradeoffs}. This approach forces designers to directly confront how their algorithm couples fairness coordination with congestion signaling. With a well-reasoned contract established, designers can then implement effective dynamics using the principles outlined in Section~\ref{sec:canonical}.

The contracts framework offers several key benefits over traditional NUM approaches:

\begin{itemize}
\item It provides more actionable guidance that matches how congestion control algorithms are actually built in practice
\item It encapsulates intertwined performance metrics in a memorable, intuitive way
\item It helps systematize the design space, potentially reducing redundant work on algorithms that merely reinvent existing points in this space
\end{itemize}

In Sections~\ref{sec:pitfalls} and below, we detail specific design pitfalls that our contracts-based approach helps identify and avoid. While no framework can anticipate all possible mistakes, we believe our approach addresses the most common and consequential design errors in congestion control.


To accommodate the diversity of congestion control algorithms—which encode
information in various signal properties, such as magnitude (e.g., delay) or
statistical moments (e.g., loss rate)—our contract definition provides
flexibility in selecting \s. However, this freedom must be exercised
judiciously. Consider Vegas: while mathematically equivalent, defining $\s =
\delay^2$ with $\func(\s) = 1/\sqrt{\s}$ unnecessarily complicates
interpretation compared to the more intuitive choice of $\s = \delay$ with
$\func(\s) = 1/\delay$. Both representations yield identical performance
properties, but the latter allows more direct mapping between our analytical
results and physical quantities, eliminating an additional translation step.
This principle of selecting the most natural representation for \s improves
both clarity and practical applicability of our analysis.


\subsection{Motivation and Common Design Pitfalls}

While the philosophy of contracts shares similarities with Network Utility Maximization (NUM)~\cite{num-kelly, num-srikant, num-low, duality-vegas}, we believe our formulation offers a more intuitive framework that aligns with how the congestion control community approaches algorithm design. Despite the mathematical foundations being well-established, we observe that many CCA designs—including recent proposals—repeatedly commit avoidable mistakes that result in poor performance.

We argue that CCA design should begin by explicitly selecting a contract, which forces designers to reason about the fundamental coupling between fairness coordination and congestion. This approach naturally guides designers to consider the tradeoffs described in Section~\ref{sec:metrics-tradeoffs} rather than myopically optimizing individual metrics (e.g., minimizing latency without considering fairness implications). Once an appropriate contract is selected, designers can implement suitable dynamics following considerations in Section~\ref{sec:canonical}.

Below, we highlight several common design pitfalls that our contracts-based approach helps avoid:

\myparagraph{Mistake \#1: Absence of a Contract} 
CCAs like TIMELY~\cite{timely} lack a well-defined contract, meaning there is no unique mapping between steady-state rate and congestion signals. As demonstrated in~\cite{ecn-vs-delay}, TIMELY's steady-state equations admit infinitely many solutions, each corresponding to different rate allocations (provided they sum to link capacity). This fundamental flaw can result in arbitrary unfairness among competing flows.

\myparagraph{Mistake \#2: Selecting Extreme Contracts} 
Proposals such as ICC~\cite{icc} and the exponential CCA from~\cite{starvation} optimize for a narrow subset of performance metrics, leading to contracts that excel in limited dimensions but perform poorly in others. These designs typically cause extreme unfairness in multi-bottleneck topologies, and in ICC's case, exhibit significant brittleness to noise in congestion signals (Section~\ref{sec:metrics-tradeoffs}).

\myparagraph{Mistake \#3: Suboptimal Dynamics and Implementation}
Many CCAs employ suboptimal dynamics to implement their contracts. For instance, Swift~\cite{swift} uses AIMD for congestion window updates despite having an explicit contract. With a properly defined contract, MIMD updates can achieve exponentially fast convergence to fairness while maintaining stability (Section~\ref{sec:canonical}). As illustrated in Figure~\ref{fig:reno-contract}, flows compute the same target rate when measuring identical loss rates, and can converge to this common rate using various update mechanisms—flows have no incentive to change their rates only when all rates equal both each other and the target rate.

Similarly, PowerTCP~\cite{powertcp} incorrectly claims inherent reactivity advantages for gradient-based approaches over traditional congestion signals. Our analysis demonstrates that reactivity characteristics are orthogonal to signal choice, and that "voltage-based" approaches can achieve equivalent convergence properties with proper implementation.

\myparagraph{Mistake \#4: Conflating Implementation with Contract}
Works like Poseidon~\cite{poseidon} artificially distinguish between AIMD control and "target scaling" (contracts), though they are mathematically equivalent approaches—AIMD implicitly creates a contract mapping between rate and congestion, while target scaling makes this relationship explicit.

\myparagraph{Mistake \#5: Overlooking Contract Implications of Minor Design Choices}
Seemingly similar algorithms like MPRDMA~\cite{mprdma}, DCTCP~\cite{dctcp}, and Reno~\cite{reno} all implement AIMD control on binary feedback signals. However, subtle implementation differences result in substantially different contracts: Reno uses "$\x = 1/\sqrt{\s}$", DCTCP uses "$\x = 1/\s^2$", and MPRDMA uses "$\x = 1/\s$". These variations lead to significantly different steady-state behaviors, as detailed in Section~\ref{sec:metrics-tradeoffs}.

Additional pitfalls are discussed in Section~\ref{sec:pitfalls}.



Our validation focuses on demonstrating negative results---fundamental
tradeoffs that cannot be avoided. If these tradeoffs exist in controlled
simulations with additional advantages given to CCAs, they will certainly
manifest in real-world networks. We choose packet-level simulations over
emulation or testbeds for two primary reasons:

First, simulations provide precise control over noise. We observed that CCAs
often perform worse than theoretically predicted due to ambient noise in
emulation or due to misestimating RTprop. By using simulations, we can isolate
specific sources of tradeoffs and even provide CCAs with oracular knowledge of
RTprop to eliminate estimation effects. This approach helps demonstrate that
the contract-based tradeoffs are truly fundamental, rather than artifacts of
implementation challenges. While RTprop estimation varies across CCAs (Vegas
never explicitly drains queues, while Copa and BBR do to estimate RTprop
accurately), and some algorithms like Swift are designed for data-center
environments where link capacity and RTprop may be known, our results show that
no CCA can overcome the fundamental limitations imposed by contracts.

Second, simulations ensure consistent algorithm availability. Not all CCAs have
Linux kernel implementations---Swift, for example, natively exists in htsim. By
using simulations, we can evaluate a comprehensive set of congestion control
approaches under identical conditions.




\section{Canonical CCA Implementation Based on Contracts}
\label{sec:canonical}

A contract can be formulated in terms of either rate or \cwnd, independent of the CCA's operational mechanism. This distinction is important as we can implement, for example, a \cwnd-based CCA utilizing a rate-based contract. While a contract determines steady-state performance, the implementation approach significantly affects dynamics, stability, and convergence time.

\myparagraph{Implementation Approaches} Various CCAs implement the same contract through different update mechanisms:
\begin{itemize}
    \item Vegas employs AIAD (Additive Increase, Additive Decrease)
    \item Swift uses AIMD (Additive Increase, Multiplicative Decrease)
    \item Poseidon implements MIMD (Multiplicative Increase, Multiplicative Decrease) with rate ratio
    \item Copa utilizes additive factors that intensify when consecutive updates maintain direction
    \item FAST TCP applies a specialized MIMD variant using RTT ratio
\end{itemize}

\begin{figure}
  \centering
  \includegraphics[]{figures/ideal_phase_portrait_all.pdf}
  \caption{State trajectory comparison under different dynamics, demonstrating how MIMD using RTT ratio achieves greater stability than alternatives based on rate ratio or delay ratio.}
  \label{fig:dynamics}
\end{figure}

\myparagraph{Contract Interpretation and MIMD Implementation} A contract such as $\rate = 1/\delay^2$ can be interpreted in two ways:
\begin{enumerate}
    \item \textbf{Target rate} as a function of \textbf{current delay}:\\ $\texttt{target\_rate} = 1/\texttt{current\_delay}^2$
    \item \textbf{Target delay} as a function of \textbf{current rate}:\\ $\texttt{target\_delay} = 1/\sqrt{\texttt{current\_rate}}$
\end{enumerate}
where $\texttt{current\_rate} = \cwnd/\rtt$ and $\texttt{current\_delay} = \rtt - \min \rtt$.

These interpretations yield two natural MIMD update mechanisms:
\begin{align}
  & \text{(1) } \tcwnd \gets \cwnd \frac{\texttt{target\_rate}}{\texttt{current\_rate}} \quad
  \text{(2) } \tcwnd \gets \cwnd \frac{\texttt{target\_delay}}{\texttt{current\_delay}}\\
  & \cwnd \gets (1-\cwndupdateavg) \cdotp \cwnd + \cwndupdateavg \cdotp \tcwnd
\end{align}

For contracts other than ``\rate = 1/\delay'', these approaches produce different dynamics, and both achieve stability only with specific values of \cwndupdateavg and network parameters (link capacity, flow count).

\myparagraph{Stability Analysis and Optimal Approach} Traditional methods exhibit significant limitations:
\begin{itemize}
    \item AIMD/AIAD mechanisms sacrifice optimal convergence time
    \item Copa's velocity mechanism generates convex rather than concave \cwnd adjustments (\eg, ETC~\cite{etc-atc}), resulting in overshoots by continuously increasing update magnitude even near convergence
    \item Poseidon's MIMD creates instability dependent on network parameters
\end{itemize}

We contend that TCP FAST's approach offers superior contract implementation. Using RTT ratio for MIMD provides enhanced stability without requiring specific \cwndupdateavg values:
\begin{align}
    & \cwnd \gets \cwnd \cdot \frac{\min \rtt + \texttt{target\_delay}}{\min \rtt + \texttt{current\_delay}}
\end{align}

Conceptually, this update recognizes that \cwnd represents ``packets in queue + packets in pipe,'' isolating the queueing delay component and scaling only this portion. This can also be interpreted as: $\cwnd \gets \rate * \textcolor{blue}{\texttt{target}\_\texttt{RTT}} = \cwnd/\rtt * \textcolor{blue}{(\min \rtt + \texttt{target\_delay})}$.

\autoref{fig:dynamics} illustrates the stability advantages of FAST's MIMD implementation compared to alternative approaches.

\myparagraph{Practical Considerations} The target RTT depends on the relationship between the target aggregate statistic and RTT. For RED-based ECN, this becomes: ``$\min \rtt + (K_{min} + (K_{max} - K_{min}) * \texttt{target\_ECN\_rate})/\bw$''. This formulation works directly in data centers where link capacity \bw is known; in other contexts, capacity must be estimated, or one must employ delay or ratio ratio with a \cwndupdateavg calibrated for the desired range of network parameters.



\section{Canonical CCA given a contract}

\label{sec:canonical}

\begin{figure}
  \centering
  \includegraphics[]{figures/ideal_phase_portrait_all.pdf}
  \caption{State trajectory under different dynamics. MIMD using RTT ratio demonstrates greater stability than MIMD using rate ratio or delay ratio.}
  \label{fig:dynamics}
\end{figure}

A contract function can be expressed in terms of either rate or \cwnd, independent of how the CCA itself operates. For instance, we can implement a \cwnd-based CCA that employs a rate-based contract. Here, we focus on \cwnd-based implementations of \rate-based contracts, though similar principles apply to other combinations.

Multiple approaches exist for implementing a CCA (\ie, \cwnd updates) given a contract. While the contract determines steady-state performance, different implementations yield varying dynamics in terms of stability and convergence time. For example, Vegas implements AIAD, Swift employs AIMD, Poseidon uses MIMD with rate ratio, Copa utilizes additive increase/decrease factors that intensify when subsequent \cwnd updates maintain direction, and FAST TCP implements a specialized form of MIMD using RTT ratio.

We contend that TCP FAST's approach offers superior contract implementation. Traditional AIMD/AIAD mechanisms sacrifice optimal convergence time, while Copa's velocity mechanism generates convex rather than concave (\eg, ETC~\cite{etc-atc}) \cwnd adjustments, resulting in overshoots. Notably, Copa continues increasing its update magnitude even when approaching convergence, whereas ideal behavior would dampen updates near convergence. Poseidon's MIMD implementation creates instability dependent on network parameters. In contrast, FAST's update mechanism ensures stability while achieving exponentially fast convergence to both fair and efficient rate allocations.

\autoref{fig:dynamics} illustrates the stability issues with vanilla MIMD and demonstrates how FAST's MIMD implementation resolves these problems.

\myparagraph{MIMD using rate or delay ratios} A contract (\eg, $\rate = 1/\delay^2$) can be interpreted in two ways: (1) \textbf{target rate} as a function of \textbf{current delay} ($\texttt{target\_rate} = 1/\texttt{current\_delay}^2$), or (2) \textbf{target delay} as a function of \textbf{current rate} ($\texttt{target\_delay} = 1/\sqrt{\texttt{current\_rate}}$), where $\texttt{current\_rate} = \cwnd/\rtt$ and $\texttt{current\_delay} = \rtt - \min \rtt$.

These interpretations yield two natural MIMD updates for implementing a contract:
\begin{align}
  & \text{(1) } \tcwnd \gets \cwnd \frac{\texttt{target\_rate}}{\texttt{current\_rate}} \quad
  \text{(2) } \tcwnd \gets \cwnd \frac{\texttt{target\_delay}}{\texttt{current\_delay}}\\
  & \cwnd \gets (1-\cwndupdateavg) \cdotp \cwnd + \cwndupdateavg \cdotp \tcwnd
\end{align}

Beyond the specific contract ``\rate = 1/\delay'', rate and delay ratios differ, producing distinct dynamics. Both approaches achieve stability only for specific values of \cwndupdateavg and network parameters (\eg, link capacity, flow count).

\myparagraph{MIMD using RTT ratio} Since we're updating \cwnd, we must determine how \rate and \delay relate to \cwnd and adjust accordingly. The following update achieves enhanced stability without requiring a specific \cwndupdateavg value:
\begin{align}
    & \cwnd \gets \cwnd \cdot \frac{\min \rtt + \texttt{target\_delay}}{\min \rtt + \texttt{current\_delay}}
\end{align}

Conceptually, \cwnd represents ``packets in queue + packets in pipe.'' This update isolates the queueing delay component, scaling only this portion using the delay ratio. Alternatively, this can be interpreted as: $\cwnd \gets \rate * \textcolor{blue}{\texttt{target}\_\texttt{RTT}} = \cwnd/\rtt * \textcolor{blue}{(\min \rtt + \texttt{target\_delay})}$.

The target RTT depends on the relationship between the target aggregate statistic and RTT. For RED-based ECN, the target RTT becomes: ``$\min \rtt + (K_{min} + (K_{max} - K_{min}) * \texttt{target\_ECN\_rate})/\bw$''. This works directly in data centers where link capacity \bw is known; otherwise, capacity must be estimated, or one must employ delay or ratio ratio with a \cwndupdateavg value calibrated for the desired range of network parameters.



\myparagraph{Avoid fixed thresholds at end-hosts} We demonstrate that fixed thresholds at end-hosts can cause starvation through an examination of AIMD on delay (as opposed to loss). This CCA was proposed in \cite{starvation} as a non-delay convergent approach to circumvent their impossibility result and appears in CCA proposals~\cite{strack, smartt} currently under consideration for standardization by the Ultra Ethernet Consortium~\cite{uec}.

AIMD on delay functions similarly to Reno (AIMD on loss), implementing additive increments when delay falls below a fixed threshold and multiplicative decrements otherwise. Consequently, its contract resembles Reno's: ``$1/\sqrt{s}$'', where $s$ represents \emph{high-delay probability} (or bytes between high-delay events) instead of \emph{loss probability}. The fixed delay threshold creates a critical problem: end-hosts disagree about when delay is high. \autoref{fig:starvation-aimd-delay} illustrates this issue in a parking lot topology where flow $f_0$ receives congestion signals from two hops. While delays experienced by flows $f_1$ and $f_2$ oscillate between the delay threshold and half this value (shown in \textcolor{TextGray}{gray}), from $f_0$'s perspective, the delay consistently exceeds the threshold. Consequently, $f_0$ never increments its \cwnd and starves.

This starvation issue can be resolved in two ways: (1) replacing fixed thresholds with dynamic ones that scale with rate—as implemented in Swift with its target delay threshold—which transforms the contract to use \delay instead of high-delay probability; or (2) relocating thresholds from end-hosts to links, as seen in Reno where packet drops occur when delay crosses a threshold at links, and in DCTCP which similarly uses ECN.

We posit that this vulnerability exists in any CCA employing fixed end-to-end thresholds for rate adjustment decisions, such as BBRv3 with $\texttt{BBRLossThresh}=2\%$~\cite{bbr-ietf}. Note the crucial distinction: Reno's threshold of ``whether loss happened'' is determined by links, whereas a threshold of ``whether loss rate exceeds 2\%'' is determined by end-hosts.



\myparagraph{Avoid fixed thresholds at end-hosts} We demonstrate that fixed thresholds can cause starvation through an examination of AIMD on delay (as opposed to loss). This CCA was proposed in \cite{starvation} as a non-delay convergent approach to circumvent their impossibility result. The same mechanism appears in CCA proposals~\cite{strack, smartt} currently under consideration for standardization by the Ultra Ethernet Consortium~\cite{uec}.


AIMD on delay functions similarly to Reno (AIMD on loss), implementing additive increments when delay falls below a fixed threshold and multiplicative decrements when exceeding it. Consequently, its contract resembles Reno's: ``$1/\sqrt{s}$'', where $s$ represents high-delay probability (or bytes between high-delay events). The critical issue stems from the fixed threshold, which causes end-hosts to disagree about when delay is high. \autoref{fig:starvation-aimd-delay} illustrates this problem in a parking lot topology where flow $f_0$ receives congestion signals from two hops. The delays experienced by flows $f_1$ and $f_2$ oscillate between the delay threshold and half this value (shown in \textcolor{TextGray}{gray}), while flow $f_0$ consistently experiences delays above the threshold. As a result, $f_0$ never increments its \cwnd and starves.

This issue can be resolved by: (1) implementing a dynamic threshold that scales with rate, as in Swift, which transforms the contract to be in terms of \delay rather than high-delay probability; or (2) relocating high-delay thresholds from hosts to links, allowing links to communicate high-delay events to hosts through mechanisms like ECN marks or packet drops.

This problem potentially affects any CCA employing fixed end-to-end thresholds to determine rate adjustments, such as BBRv3 with its $\texttt{BBRLossThresh}=2\%$~\cite{bbr-ietf}.


==> sections/design.tex <==
%-------------------------------------------------------------------------------
\section{Floating Figures and Lists}
\label{sec:design}
\label{sec:figs}
%-------------------------------------------------------------------------------

%---------------------------
\begin{figure}
\begin{center}
\begin{tikzpicture}
  \draw[thin,gray!40] (-2,-2) grid (2,2);
  \draw[<->] (-2,0)--(2,0) node[right]{$x$};
  \draw[<->] (0,-2)--(0,2) node[above]{$y$};
  \draw[line width=2pt,blue,-stealth](0,0)--(1,1)
        node[anchor=south west]{$\boldsymbol{u}$};
  \draw[line width=2pt,red,-stealth](0,0)--(-1,-1)
        node[anchor=north east]{$\boldsymbol{-u}$};
\end{tikzpicture}
\end{center}
\caption{\label{fig:vectors} Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. Text size inside figure should be as big as
  caption's text. }
\end{figure}
%% %---------------------------


Here's a typical reference to a floating figure:
Figure~\ref{fig:vectors}. Floats should usually be placed where latex
wants then. \autoref{fig:vectors} is centered, and has a caption
that instructs you to make sure that the size of the text within the
figures that you use is as big as (or bigger than) the size of the
text in the caption of the figures. Please do. Really.

In our case, we've explicitly drawn the figure inlined in latex, to
allow this tex file to cleanly compile. But usually, your figures will
reside in some file.pdf, and you'd include them in your document
with, say, \textbackslash{}includegraphics.

Lists are sometimes quite handy. If you want to itemize things, feel
free:

\begin{description}

\item[fread] a function that reads from a \texttt{stream} into the
  array \texttt{ptr} at most \texttt{nobj} objects of size
  \texttt{size}, returning returns the number of objects read.

\item[Fred] a person's name, e.g., there once was a dude named Fred
  who separated usenix.sty from this file to allow for easy
  inclusion.
\end{description}

\noindent
The noindent at the start of this paragraph in its tex version makes
it clear that it's a continuation of the preceding paragraph, as
opposed to a new paragraph in its own right.
\authA{Comment by author A.} \authB{Comment by author B.}

\subsection{LaTeX-ing Your TeX File}
%-----------------------------------

People often use \texttt{pdflatex} these days for creating pdf-s from
tex files via the shell. And \texttt{bibtex}, of course. Works for us.
